Effective Sampling for Robot Motion Planning Through the Lens of Lattices

Sampling-based methods for motion planning, which capture the structure of the robot's free space via (typically random) sampling, have gained popularity due to their scalability, simplicity, and for offering global guarantees, such as probabilistic completeness and asymptotic optimality. Unfortunately, the practicality of those guarantees remains limited as they do not provide insights into the behavior of motion planners for a finite number of samples (i.e., a finite running time). In this work, we harness lattice theory and the concept of $(\delta,\epsilon)$-completeness by Tsao et al. (2020) to construct deterministic sample sets that endow their planners with strong finite-time guarantees while minimizing running time. In particular, we introduce a highly-efficient deterministic sampling approach based on the $A_d^*$ lattice, which is the best-known geometric covering in dimensions $\leq 21$. Using our new sampling approach, we obtain at least an order-of-magnitude speedup over existing deterministic and uniform random sampling methods for complex motion-planning problems. Overall, our work provides deep mathematical insights while advancing the practical applicability of sampling-based motion planning.

==> tex/3_main_theories.tex <==
\section{Sample Complexity}\label{sec:sample_comlpexity}
We present our main theoretical results on sample complexity. First, we adapt Verger-Gaugry's~\cite{verger2005covering} lower bound result to obtain a new lower bound on the sample complexity of \decomp sets. Notice that this bound applies to any sample set, not necessarily a lattice-based one.

\begin{thm}[Sample-complexity lower bound~\protect{\cite[Theorem~3.10]{verger2005covering}}]
    Consider the configuration space $\C$ being a $d$-dimensional R-ball\itai{change here}, $\B_R\subset \dR^d$. Without loss of generality, assume\footnote{These radius ranges are assumed so that they fit into the setting of a theorem we use later.} $R=\sqrt{d}\beta$ or $R\geq d\cdot\beta$, where $\beta:=\beta\left(\delta,\epsilon\right)$ as defined in Lemma 1. Suppose that $\X$ is a sample set that is a $\beta$-cover for $\C$. Then there exists $c>0$ such that:
    \[
        |\X|\geq cd\left(\frac{R}{\beta\left(\de\right)}\right)^d =: n_{LB}^{\de}.
    \]
    % \triangleq \|\X_{LB}\|
\end{thm}
\begin{proof}
Theorem 3.10 in~\cite{verger2005covering} states that if a sample set $\X^*$ is a $\frac{1}{2}$-cover for $\B_{R^*}$, where $R^*=\frac{\sqrt{d}}{2}$ or $R^*\geq\frac{d}{2}$, then there exists $c>0$ such that $|\X^*|\geq cd\cdot \left(2R^*\right)^d$.


Next, we use a rescaling argument to apply those finding to our setting. In particular, we wish to cover $\B_R$ with $\beta$-balls. To convert $\beta$-balls into $\frac{1}{2}$-balls we need to rescale by $\frac{1}{2\beta}$, which makes it so that $R$ becomes $R^*=\frac{R}{2\beta}$ in the rescaled space. In this rescaled space, $\B_{R^*}$ is covered by $\frac{1}{2}$-balls. 


For the radius $R^*$ to fit Verger-Gaugry's requirements we need to ensure  that:
\begin{equation*}
    \frac{R}{2\beta} = R^* = \frac{\sqrt{d}}{2},
\end{equation*}
which implies that:
\[
    R=\sqrt{d}\beta,
\]
and similarly if \footnote{Notice that this lower bound applies to any ball $\B_r$, as long as it is $\sqrt{d}$ times or more than $d$-times the "minimal radius" ball of $\beta$.} $R\geq d\beta$. I want to demonstrate next why we can safely assume that our C-Space's radius is $\sqrt{d}$-times the radius of the $\beta$-ball. \itai{new segment here}


Taking $d=10$ for example, if our space's radius is $\sqrt{10}$ times bigger than a $\beta$-ball then the volume is $\sqrt{10}^{10}=10^5$ bigger than a $\beta$-ball. This means we expect to find about $10^5$ smaller $\beta$-balls in it. With a normal cubic $[0,1]^d$ world, we expect to find about $\frac{1}{\beta^d}=\left(\frac{1}{\beta}\right)^d=\left(\frac{1}{\beta^2}\right)^{\frac{d}{2}}$ balls. Taking the same $d=10$, we get that for our spherical space to have less $\beta$-balls than a cubic space, we will need $\frac{1}{\beta^2}\geq 10 \Rightarrow \beta \leq 0.32$. We get:
\[
    \beta=\delta\sqrt{\frac{\epsilon^2}{1+\epsilon^2}}\leq0.32 \iff \frac{\epsilon^2}{1+\epsilon^2}\leq \left(\frac{0.32}{\delta}\right)^2
\]
But notice that:
\[
    \frac{0.32}{\delta}<1 \iff \delta>0.32
\]
So for $\delta\leq 0.32$, we get $\frac{0.32}{\delta}\geq1$. But $\frac{\epsilon^2}{1+\epsilon^2}<1$ for all $\epsilon>0$, which makes the above inequality true for all $\epsilon>0$. All this is to say the following: the requirements on $\delta,\epsilon$ aren't harsh and would probably be fulfilled in most use cases, allowing us to rely on this lower bound. Returning to Verger-Gaugry's result, we get the lower bound:
\begin{equation*}
    |\X|\ \geq cd\cdot \left(2R^*\right)^d = cd\cdot \left(\frac{R}{\beta}\right)^d,
\end{equation*}
which concludes the proof. \qedsymbol
\end{proof}
\itai{Note to self: either remove the following part or find a suitable comparison between square and spherical CSpaces.}


\itai{I moved this section HERE, Im not sure why it was down below.}
Let us compare this lower-bound to a more naive bound, asserting the minimal number of points in a set $\X_{base}$ should be at least the volume of $\B_R$ divided by the volume of a $\beta$-ball:
\begin{equation}
        |\X_{base}|\geq \frac{Vol\left(\B_R\right)}{Vol\left(\B_\beta\right)}=\frac{c_d R^d}{c_d\beta^d}=\left(\frac{R}{\beta}\right)^d.
\end{equation}
It is immediately clear that the new lower bound is $d$ times better than the classic one. This is another reason to support spherical configuration spaces.

Next, we will define what is a "lattice sample set" and show that we can give explicit representations of them such that they'll be \decomp sets. As we will be talking about covering the space throughout the paper, let us first consider the following definition from Conway and Sloane~\cite{conway2013sphere}:
\begin{definition} (Covering Radius)
    \itai{changes here} For a collection of points $\X$, a covering radius is defined to be:
    \[
        R_{cover}^{\X} = \sup_{y\in\mathbb{R}^d}\inf_{x\in\X} \|x-y\|.
    \]
\end{definition}
\itai{added some clarification here}
This definition makes it more clear that one can not cover $\mathbb{R}^d$ with a radius smaller than $R_{cover}^{\X}$ for a given point set $\X$. In the next theorem, we will be using the covering radii's optimality to construct $\beta$-balls, paving the way to explicitly construct \decomp sample sets.
% \begin{lemma}[Optimal covering radius]
%     Let $\Lambda$ be a lattice in $\mathbb{R}^d$. Then $Cover\left(\Lambda\right)$ is the optimal \left(in terms of density\right) covering radius for this $d$-dimensional lattice. Relying on Conway~\cite{conway2013sphere}, we have:
%     \itai{I'm correcting this. the optimal radius is related to the original lattice, not the rescaled one.}
%     \begin{enumerate}[topsep=1pt,itemsep=1ex,partopsep=1ex,parsep=1ex]
%         \item $Cover\left(\AN\right) = \sqrt{\frac{d}{2}}$
%         \item $Cover\left(\DN\right) = \frac{\sqrt{d}}{2}$
%         \item $Cover\left(\ZN\right) = \sqrt{\frac{d\left(d+2\right)}{12\left(d+1}}$
%     \end{enumerate}
% \end{lemma}
% \itai{changes here.}
% Using the concept of covering radii for lattices, we will explicitly find sample sets defined by our three lattices:
% \begin{definition}[Lattice Sample Set]
%     Let $\Lambda$ be a lattice, and $\delta,\epsilon$ be the clearance and stretching parameters. We define $\XL$ to be the set $\left(c\cdot\Lambda\right)$ for some $c>0$ such that it's a \decomp set.
% \end{definition}
% Specifically for \Lattices we get the following theorem:
\begin{thm}
  Fix $\delta>0,\epsilon>0$. Then the following sets are \decomp:
  \itai{added a new case for Dn (even/odd)}
  \begin{enumerate}
      \item $\XZ=\frac{2\beta\left(\delta,\epsilon\right)}{\sqrt{d}}\ZN$,
      \item $\XD=
      \begin{cases}
        d\text{ is odd: }
        \{x\in\mathbb{R}^d|x=\frac{4\beta\left(\delta,\epsilon\right)}{\sqrt{2d-1}}G_{\DN}^t\cdot v,v\in\mathbb{Z}^d\}:=\frac{4\beta\left(\delta,\epsilon\right)}{\sqrt{2d-1}}\DN,\\
        d\text{ is even: }
        \{x\in\mathbb{R}^d|x=\sqrt{\frac{8}{d}}\beta G_{\DN}^t\cdot v,v\in\mathbb{Z}^d\}:=\sqrt{\frac{8}{d}}\beta\DN,
      \end{cases}$
      \item $\XA=\{\mathbb{R}^d|x=\sqrt{\frac{12\left(d+1\right)}{d\left(d+2\right)}}\beta\left(\delta,\epsilon\right) T\cdot v,v\in\mathbb{Z}^d\}:=\sqrt{\frac{12\left(d+1\right)}{d\left(d+2\right)}}\beta\left(\delta,\epsilon\right) T(\AN)$,
      
      
      with:
      $T=\begin{pmatrix}
                    1 &  1  & \dots & 1 & x - 1\\
                    -1 & 0  & \dots & 0 & x \\
                    0 & -1  & \dots & 0 & x \\
                    \vdots & \vdots  &  \ddots & \vdots & \vdots \\
                    0 & 0  &  \dots & -1 & x \\
                \end{pmatrix}\in \mathbb{R}^{d \times d}, x=\frac{1}{(d+1) - \sqrt{d+1}}$.
  \end{enumerate}
\end{thm}
\begin{proof}
    \itai{this section onwards has changes} We need to show that we can rescale the lattices \Lattices by some $c>0$ such that they become \decomp. We remember that the lattices were introduced in the first section in the context of using unscaled distances---i.e., in a cube $[0,1]^d$ we have exactly one cube for the lattice $\mathbb{Z}^d$, in contrast with many more cubes if we start rescaling the grid. Since we want the samples to be sufficiently dense as to form a \decomp set, we will need to rescale the space. This is why in each of the following sections, given our lattice $\Lambda$, we use a \emph{rescale coefficient} $f_\Lambda:=f_\Lambda\left(d\right)$, together with a \emph{rescaling factor} $w_\Lambda>0$, defined by:
    \[
        \beta = f_\Lambda w_\Lambda\Rightarrow w_\Lambda = \frac{\beta}{f_\Lambda}.
    \]
    Meaning: we start with the covering radius (i.e. the rescale coefficient $f_\Lambda$), and we rescale it (i.e. multiply it with the rescaling factor) to "the smallest size possible" (i.e. the $\beta$-ball that covers the space), which is sufficient for $\left(\delta,\epsilon\right)$-completeness due to Lemma~\ref{lem:cover}.
    One thing to note is, that using our scaling equation, our space went from some implicit "originating" space of radius $R_{orig}$ (where, as we said, the lattices are still unscaled)---which becomes $R$ with the relation:
    \begin{align*}
        R_{orig}\cdot w_\Lambda = R \Rightarrow \frac{R_{orig}\cdot\beta}{f_\Lambda}=R\Rightarrow R_{orig}=\frac{R}{\beta}\cdot f_\Lambda.
    \end{align*}
    We will find $f_\Lambda$ for each of our three lattices, which will immediately give us our \decomp sets.


    \itai{This whole section was overhauled (no more enumerate, rewritten, etc.)} We first look at $\ZN$. Consider the cube $[0,w_{\ZN}]^d$ which tessellates the space. To find the rescale coefficient, remember that we need to completely cover each of these lattice cubes. Thus, the radius needs to reach the center of the cube. Seeing as the cube has a side of length $w_{\ZN}$, this gives us the scaling equation:
    \[
        \beta = \frac{\sqrt{d}}{2}w_{\ZN} \Rightarrow f_{\ZN}\left(d\right)=\frac{\sqrt{d}}{2},
    \]
    from which we get our set definition:
    \begin{align*}
        \XZ = \{x\in\mathbb{R}^d|x=w_{\ZN} v\cdot G_{\ZN},v\in\mathbb{Z}^{1\times d}\} = \\
        \{x\in\mathbb{R}^d|x=\frac{\beta}{f_{\ZN}\left(d\right)}I_{d\times d}\cdot v,v\in\mathbb{Z}^d\} = \\
        \{x\in\mathbb{R}^d|x=\frac{2\beta}{\sqrt{d}} v,v\in\mathbb{Z}^d\}:=\frac{2\beta}{\sqrt{d}}\ZN.
    \end{align*}
    Next, we look at $\DN$. Here we use the fact that the covering radius for $D_{d\text{-odd}}^*$ is \(\frac{\sqrt{2d-1}}{4}\), and for $D_{d\text{-even}}^*$ is \(\frac{\sqrt{2d}}{4}=\sqrt{\frac{d}{8}}\) (~\cite[page 120]{conway2013sphere}). Using this radius as a baseline for what we want our $\beta$-ball to be, we get the following rescaling equations:
    \begin{align*}
                \beta = \frac{\sqrt{2d-1}}{4}w \Rightarrow f_{D_{d\text{-odd}}^*}\left(d\right) = \frac{\sqrt{2d-1}}{4}, \\
                \beta = \sqrt{\frac{d}{8}}w \Rightarrow f_{D_{d\text{-even}}^*}\left(d\right) = \sqrt{\frac{d}{8}},
    \end{align*}
    from which we get our set definitions:
    \begin{align*}
        D_{d\text{-odd}} = \{x\in\mathbb{R}^d|x=wv\cdot G_{\DN},v\in\mathbb{Z}^{1\times d}\} = \\
        \{x\in\mathbb{R}^d|x=\frac{4\beta}{\sqrt{2d-1}}G_{\DN}^t\cdot v,v\in\mathbb{Z}^d\}:=\\
        \frac{4\beta}{\sqrt{2d-1}}\DN,\\
        D_{d\text{-even}} = \{x\in\mathbb{R}^d|x=wv\cdot G_{\DN},v\in\mathbb{Z}^{1\times d}\} = \\
        \{x\in\mathbb{R}^d|x=\sqrt{\frac{8}{d}}\beta G_{\DN}^t\cdot v,v\in\mathbb{Z}^d\}:=\\
        \sqrt{\frac{8}{d}}\beta\DN.
    \end{align*}
    Finally, we analyze the lattice $\AN$.
    % Using a lattice's generator, we can define the lattice points generated from it as:
    % \[
    %     \Lambda=\{x \in \mathbb{R}^{d} \mid \exists g\in \mathbb{Z}^{d} \text{ s.t. } x=g\cdot G\}
    % \]
    Recall that $A_d^*$ is defined using this \emph{generator matrix}:
    \begin{align} \label{eq:generaror}
        G:=G_{\AN}=
        \begin{pmatrix}
            1 & -1 & 0 & 0 & \dots & 0 & 0 \\
            1 & 0 & -1 & 0 & \dots & 0 & 0 \\
            . & . & . & . & \dots & . & 0 \\
            1 & 0 & 0 & 0 & \dots & -1 & 0 \\
            \frac{-d}{d+1} & \frac{1}{d+1} & \frac{1}{d+1} & \frac{1}{d+1} & \dots & \frac{1}{d+1} & \frac{1}{d+1} \\
        \end{pmatrix}\in \mathbb{R}^{d\times \left(d+1\right)}.
    \end{align}
    As this is a mapping from $d$ to $d+1$, we start with the process of embedding $A_d^*$ in $\mathbb{R}^d$. Afterwards we show that the embedding we created in $\mathbb{R}^d$ shares the same covering radius as the original set in $\mathbb{R}^{d+1}$.

    
    Notice that the rows of $G$ are all in the plane $H_0: \sum_i x_i = 0$, so $A_d^*$ itself is contained in that $d$-dimensional plane. It remains to find a transformation of $\AN$ such that the dimension is reduced to $d$, while maintaining the structure of the points in $\AN$.
    
    
    First, we will rotate $H_0$ so that we zero out the last coordinate. To do that, we will use a \emph{Householder matrix}~\cite{householder1958unitary}, which gives us a way to reflect a point set with a plane. Defining the plane through its normal vector $\hat{n}\in \mathbb{R}^{d+1}$, the Householder matrix is defined as:
    \begin{align}\label{eq:reflection}
        P=I-2\hat{n}\hat{n}^t.
    \end{align}
    We need to find the normal $\hat{n}$ to a plane that is exactly between (angle-wise) the plane $H_0$ and the $X_{d+1}=0$ plane, because reflecting against this plane will give us points that lie in $X_{d+1}=0$. \itai{fixed many typos and rewritten this section. The angle thing wasnt accurate enough IMO, so I proved it another way.}
     Finding an angle between planes is equivalent to finding the angle between their normal vectors, which leads us to the following \emph{intuition} in two dimensions.
     \begin{figure}[H]
        \centering
        \includegraphics[width=0.45\linewidth]{Images/normal_inuition.jpg}
        \caption{Illustraion of finding the reflection normal in $d=2$}
        \label{fig:reflection}
    \end{figure}
     the plane $H_0$ has a normal vector $u=\left(\frac{1}{\sqrt{2}},\frac{1}{\sqrt{2}}\right)$. We want to find the vector splitting the angle between u and $(0,-1)$. We can look for it on the vertical line descending from $u$, and because $\|u\|=\|(0,-1)\|=1$ then to make sure it splits the angle we just need that 
     \begin{align*}
         n\cdot u = n\cdot (-e_2) \iff \\
         \left(\frac{1}{\sqrt{2}},\frac{1}{\sqrt{2}}-\alpha\right)\cdot\left(\frac{1}{\sqrt{2}},\frac{1}{\sqrt{2}}\right)=\left(\frac{1}{\sqrt{2}},\frac{1}{\sqrt{2}}-\alpha\right)\cdot(0,-1) \Rightarrow \\
         \frac{1}{2}+\frac{1}{2}-\alpha\frac{1}{\sqrt{2}}=\alpha-\frac{1}{\sqrt{2}} \Rightarrow \\
         1+\frac{1}{\sqrt{2}}=\alpha(1+\frac{1}{\sqrt{2}})\Rightarrow\alpha=1,
     \end{align*}
    getting the normal $n=\left(\frac{1}{\sqrt{2}},\frac{1}{\sqrt{2}}-1\right)$. It can be shown that the same idea repeats in $d=3$ with $n=\left(\frac{1}{\sqrt{3}},\frac{1}{\sqrt{3}},\frac{1}{\sqrt{3}}-1\right)$, leading us to the following generalization.
    Let $e_{d+1}=\left(0,\dots,0,1\right)\in\mathbb{R}^{d+1},u=\left(\frac{1}{\sqrt{d+1}},\dots,\frac{1}{\sqrt{d+1}}\right)\in~\mathbb{R}^{d+1}$. Define $n:=\left(-\frac{1}{\sqrt{d+1}},\dots,-\frac{1}{\sqrt{d+1}},1-\frac{1}{\sqrt{d+1}}\right)$ (this is the same as our $d=2,3$ cases, only with an opposite sign). We are now going to show that this vector, when used with the Householder matrix, will rotate $H_0$ to "the floor"---i.e. reflection onto the $[X_1,\dots,X_d]$ plane. Using $\hat{n}=\frac{n}{\|n\|}$ to get a normalized vector, we can calculate the Householder matrix, getting
    \begin{align}
        P=
        \begin{bNiceArray}{cw{c}{1cm}c|c}[margin]
            \Block{3-3}<\Large>{I_d - \frac{1}{D-\sqrt{D}}\mathds{1}} 
            & & & \dfrac{1}{\sqrt{D}} \\
            & & & \Vdots \\
            & & & \dfrac{1}{\sqrt{D}} \\
            \hline
            \dfrac{1}{\sqrt{D}} & \dots& \dfrac{1}{\sqrt{D}} & \dfrac{1}{\sqrt{D}}
        \end{bNiceArray}.
    \end{align}
    We need to show that for all $i\leq d+1$, the last element of $v=PG_{\AN}^t\cdot e_i$ is always zero. First, for all $i<d+1$, we easily get
    \begin{align*}
        PG_{\AN}^t\cdot e_i=P\cdot
        \begin{pmatrix}
            1 \\
            0 \\
            \vdots \\
            0 \\
            -1 \\
            0 \\
            \vdots \\
            0
        \end{pmatrix}.
    \end{align*}
    But, in the matrix $P$, the last elements of all $i<d+1$ columns are all equal. This means that taking $+1$ of one and $-1$ of the other will give us 0 there. We are left with $e_{d+1}$, which gives us
        \begin{align*}
        PG_{\AN}^t\cdot e_{d+1}=P\cdot
        \begin{pmatrix}
            -\frac{D-1}{D} \\
            \frac{1}{D} \\
            \vdots \\
            \frac{1}{D}
        \end{pmatrix}.
    \end{align*}
    Looking specifically at the last element, we get
    \begin{align*}
        \frac{1}{\sqrt{D}}\cdot\frac{1-D}{D} + (D-1)\frac{1}{D}\frac{1}{\sqrt{D}}=\frac{1-D+D-1}{D\sqrt{D}}=0,
    \end{align*}
    showing what we needed.
    % Let $\angle\left(u,v\right)$ denote the angle between the vectors $u,v$. Then we get that $\cos\left({\angle\left(u,n\right)}\right) = \cos\left({\angle\left(-e_{d+1},n\right)}\right)$:
    % \begin{align*}
    %     \cos\left({\angle\left(u,n\right)}\right) = \frac{u\cdot n}{\|u\|\|n\|} = \frac{\frac{-1}{d+1}\cdot d + \frac{1}{\sqrt{d+1}} - \frac{1}{d + 1}}{\|n\|} = \frac{\frac{1}{\sqrt{d+1}} - 1}{\|n\|}, \\
    %     \cos{\angle\left(\left(-e_{d+1}\right),n\right)} = \frac{\left(-e_{d+1}\right)\cdot n}{\|-e_{d+1}\|\|n\|} = \frac{\frac{1}{\sqrt{d+1}} - 1}{\|n\|},
    % \end{align*}
    % In $d=2$ the three vectors $-e_{d+1},u,n$ are on the same 3D-plane, as we have
    % \[
    %     u\times n = n \times (-e_{d+1}) = (\frac{1}{\sqrt{D}}, \frac{1}{\sqrt{D}}, 0).
    % \]
    % For three vectors $-e_{d+1},u,n$ on the same plane to define two angles that have the same cosine value, they need to have angles $\pi+x,\pi-x$. But these three unique vectors define three unique angles, and $\pi+x +\pi-x=2\pi$, which is a contradiction. This means that their angles are equal, finishing our claim for $d=2$. This serves as a motivation for defining this $n$ vector for all $d$ dimensions. I
    
    
    Using this, all we have left to do is use an embedding that ignores the last element, meaning $E:\mathbb{R}^{n+1}\Rightarrow\mathbb{R}^d$ defined by $E\left(x_1,\dots,x_d,x_{d+1}\right)=\left(x_1,\dots,x_d\right)$. We finish with the following definition that helps us explicitly calculate points in $A_d^*$ (using (\ref{eq:generaror}), (\ref{eq:reflection})):
    \begin{align}
        T: \mathbb{Z}^d\Rightarrow\mathbb{R}^d \nonumber \\
        T\left(g\right) = EPG^t\left(g\right).
    \end{align}
    \itai{a new explanation about T. }
    \begin{figure}[H]
        \centering
        \begin{subfigure}[b]{0.49\textwidth}
            \includegraphics[width=\textwidth]{Images/EPGt_visual_explanation1.png}
            \caption{Sample points in $H_0$}
            \label{fig:epgt_visual1}
        \end{subfigure}
        \hfill
        \begin{subfigure}[b]{0.49\textwidth}
            \includegraphics[width=\textwidth]{Images/EPGt_visual_explanation2.png}
            \caption{$H_0$ rotated to the "floor"}
            \label{fig:epgt_visual2}
        \end{subfigure}
        \hfill
        \begin{subfigure}[b]{0.49\textwidth}
            \includegraphics[width=\textwidth]{Images/EPGt_visual_explanation3.png}
            \caption{The samples as they look in $\mathbb{R}^2$}
            \label{fig:epgt_visual3}
        \end{subfigure}
        \caption{Lowering dimensions in $A_2^*$}
        \label{fig:egpt_visual}
    \end{figure}
    This is what the transformation does: first (Fig.~\ref{fig:epgt_visual1}), $G^t$ takes an integer vector in $\mathbb{R}^d$ and turns it to a vector in $\AN\subset\mathbb{R}^{d+1}$. Next (Fig.~\ref{fig:epgt_visual2}), $P$ takes the element in $\AN$ and reflects it into $[X_1,\dots,X_d]$---effectively lowering its dimension. Lastly (Fig.~\ref{fig:epgt_visual3}), because we are still in $\mathbb{R}^{d+1}$, we use $E$ to embed it into $\mathbb{R}^d$.
    
    \itai{changed all N to D in the following sections and changed a bit the order of things}
    Formally, we start by defining the embedding $E$. Let $D:=d+1$, then
    \begin{align*}
        E=
        \begin{pmatrix}
            1 & 0 & \dots & 0 & 0 \\
            0 & 1 & \dots & 0 & 0 \\
            . & . & \dots & . & 0 \\
            0 & 0 & \dots & 1 & 0
        \end{pmatrix},
    \end{align*}
    which, together with $P$ (in (6)), we use to calculate $EP$ 
    \begin{align*}
        \left(EP\right)^t=
        \begin{bNiceArray}{cw{c}{1cm}c}[margin]
            \Block{3-3}<\Large>{I_d - \frac{1}{D-\sqrt{D}}} 
            & &  \\
            & &  \\
            & &  \\
            \hline
            \dfrac{1}{\sqrt{D}} & \Cdots& \dfrac{1}{\sqrt{D}}
        \end{bNiceArray}\in\mathbb{R}^{d\times(d+1)}.
    \end{align*}
    From here it can be shown that
    \begin{align}
        T^t=G\left(EP\right)^t=
        \begin{pmatrix}
            1 & -1 &  0  & \dots & 0 \\
            1 & 0  &  -1 & \dots & 0 \\
            . & .  &  .  & \dots & . \\
            1 & 0  &  0  & \dots & -1 \\
            \frac{1}{D - \sqrt{D}} - 1 & \frac{1}{D - \sqrt{D}} & \frac{1}{D - \sqrt{D}} & \dots & \frac{1}{D - \sqrt{D}}
        \end{pmatrix}\in\mathbb{R}^{d\times d}
    \end{align}
    Being that reflections are isometries, and so are embeddings, we can use the same covering radius after using $T$. So, we are given the rescaling coefficient through the covering radius (~\cite[page 115]{conway2013sphere}):
    \[    
        \beta = \sqrt{\frac{d\left(d+2\right)}{12\left(d+1\right)}}w_{\AN} \Rightarrow f_{\AN}\left(d\right)=\sqrt{\frac{d\left(d+2\right)}{12\left(d+1\right)}},
    \]
    from which we get our set definition:
    \begin{align*}
        \XA = \{x\in\mathbb{R}^d|x=w_{\AN}T\cdot v,v\in\mathbb{Z}^d\} = \\
        \{x\in\mathbb{R}^d|x=\sqrt{\frac{12\left(d+1\right)}{d\left(d+2\right)}}\beta T\cdot v,v\in\mathbb{Z}^d\}\, \qedsymbol
    \end{align*} 
\end{proof}
% The above result directly follows from~\cite{verger2005covering} which provides a lower bound on the number of $\tfrac{1}{2}$-balls necessary to cover a ball of radius $R \geq \frac{d}{2}$. A simple rescaling argument is used to make it applicable to our setting where $\beta\left(\de\right)$-balls are used for covering the configuration space. \kiril{Does this description give justice to what you derived or is there something more complicated that I'm missing here?}

% This is a fair upper bound on $\beta=\delta\alpha$, as $\alpha \leq 1$ and we already take $\delta$ as small value, usually. For example, for a 10 degree problem, we would need $\beta\leq\frac{1}{6}\approx 0.17$---then for $\delta = 0.1$ we would need $\epsilon < 1.7$. \kiril{I don't understand this discussion. Please clarify.}
% NOTE \itai{I commented out all this part \left(see tex file\right). Its irrelant as I rewrote the theorem.}
% Let us compare this bound with the previous bound~\cite[Theorem~1]{tsao2020sample}, which employed volume arguments. \kiril{Is this the bound you had in mind?} In particular, the previous bound is at least 
% \kiril{please fill in.}
% Thus, the new upper bound is bigger by a factor of \kiril{fill} than the old one. 

% \kiril{The following text needs to be clarified as in the first equation the new bound is stated and I substituted it with the text above.}
% {\color{blue} To compare this LB to the "classic" volume-derived lower bound, let us return to a configuration space defined in a ball of general radius $r\geq \beta d$. \kiril{return from where? let's keep everything consistent and keep the same setting throughout the paper unless absolutely necessary.}
% We get the following lower bound:
% \begin{align}
%     n \geq k d\cdot\left(2r_0\right)^d =k\cdot d \left(\frac{r}{\beta}\right)^d 
% \end{align}
% NOTE \itai{I commented out all this part also \left(see tex file\right). To clarify: this is a comparison to the classic "volume divided by volume" lower bound, I didn't compare this lower bound to the one in tsao. you dealt with a square C-Space there and I found it hard to compare your approximation to this one.}
% \begin{proof}
%   We rely on , which states that if a sample set $\X$ is a for  then
% \begin{align}
%    |\X| \geq k\cdot d \cdot\left(2R\right)^{d},\,k>0. 
% \end{align}
% \kiril{What is the purpose of $k$? Does it hold for any $k$? If so, can we substitute $\geq$ with $>$ and get rid of $k$?}
% In our setting, we wish to construct a $\beta\left(\de\right)$-cover of our configuration space. 
% We want $\frac{1}{2}$-balls in~\cite{verger2005covering}  to be mapped to balls of radius $\beta\left(\de\right)$-balls, so we need a rescaling factor of $2\beta$. This means that if we want to cover a general ball of radius $r$ by $\beta$-balls, then we need a ball of initial radius $R$ \left(before the rescaling\right) such that:
% \[
%     R\cdot 2\beta=rarrow R=\frac{r}{2\beta}
% \]
% Taking $R\geq\frac{d}{2}$ to fit Verger's result, we reach the following bound on $r>0$:
% \begin{align*}
%     \frac{d}{2} \leq R = \frac{r}{2\beta} arrow r \geq \beta d
% \end{align*}
% To get a feeling for this bound, let us choose our configuration space as a ball of radius $r=\frac{\sqrt{d}}{2}$. This is logical because it is the circumsphere of the regular $[0,1]^d$ cube. With this we need to have:
% \[
%     \frac{\sqrt{d}}{2} \geq \beta d arrow \beta \leq \frac{1}{2\sqrt{d}}
% \]
% \end{proof}
\itai{rewritten section}
% We are now going to find new upper bounds for our newly defined sample sets \Lattices. We name an upper bound for a sample set by the name \emph{sample complexity}. 
% Throughout the analysis, we assume that the configuration space is the Euclidean $d$-dimensional $R$-ball denoted by $\B_R$. This assumption allows us to obtain tighter bounds, than for, say, unit hypercube configuration spaces, which were assumed in previous sample-complexity analysis. 
% To this end, we first introduce the \emph{Gram matrix} of a lattice, relevant to the following Theorem:
%   \begin{definition}[Gram matrix and quadratic form]
%       The \emph{Gram matrix} of a lattice $\Lambda$ with generator matrix $G_\Lambda$ is defined to be $Gr_\Lambda:=G_\Lambda G^t_\Lambda$. Additionally the quadratic form of $\Lambda$ is defined as $q_\Lambda\left(a\right):=aGr_\Lambda a^t$.
%   \end{definition}
In this next theorem, we derive analytical upper bounds for \Lattices, a property we call \emph{sample complexity}. To achieve that, we first derive an upper bound for general lattices. Later on, in our experimental results (Section~\ref{sec:experiments}), we compare the sample complexity of those sets for varying values of $\de$, and $d$. 

\begin{thm}[General lattice sample complexity]
\label{general_sample_complexity}
    Consider a lattice $\Lambda$ that defines the \decomp set $\XL$ in a C-Space $\B_R$. Recall that $\beta=\beta\left(\delta,\epsilon\right)$ is explicitly given in equation (1). Then we get the sample complexity:
    \begin{align*}
        |\XL\cap \B_R| = O\left(\frac{1}{d}\left(\left(\frac{R}{\beta}\right)^2\frac{2\pi e}{d}\cdot f_\Lambda^2\left(d\right)\right)^{\frac{d}{2}} + \left(\frac{R}{\beta}\cdot f_\Lambda\left(d\right)\right)^{d-2}\right).
    \end{align*}
\end{thm}
\begin{proof}
  We wish to estimate the size of sample set $\X_\Lambda$ induced by the lattice $\Lambda$ and the scaling factor $f_\Lambda\left(d\right)$. We first show that this is equivalent to estimating the expression $|\B_R\cap \Lambda|$. Let $v=aG_\Lambda,\,a\in\mathbb{Z}^d$ be a lattice point, then by definition of a \emph{Gram matrix} as being $Gr_\Lambda:=G_\Lambda G_\Lambda^t$, we obtain 
  \[
    aGr_\Lambda a^t:=aG_\Lambda G^t_\Lambda a^t=\|aG_\Lambda\|^2=\|v\|^2.
  \]
  This leads to the relation
  \begin{align*}
      \B_R\cap \Lambda &= \{v\in\Lambda |\,\|v\| \leq R\} =\{a\in\dZ^d|a Gr_\Lambda a^t\leq R^2\} \\ & =E_{R^2}\left(Gr_\Lambda\right)\cap \dZ^d,
  \end{align*}
  where $E_{s}\left(A\right):=\{x\in\dR^d|x A x^t\leq s\}$. 
  
  
  Next, observe that the Gram matrix $Gr_\Lambda$ of the lattices \Lattices contains only rational numbers, and hence defines what is called a \emph{"rational quadratic form"}. This allows us to use Landau's \emph{rational ellipsoid bound theorem}~\cite{ivic2004lattice} which asserts that
  \begin{equation*}
      |E_{r^2}\left(Gr_\Lambda\right)\cap \dZ^d|=\frac{\vol\left(\B_{s}\right)}{\sqrt{d}}+\Theta\left(s^{d-2}\right),
  \end{equation*}
hence,
\begin{align}\label{volume_delta}
    |\B_R\cap \Lambda|=\frac{\vol\left(\B_{R}\right)}{\sqrt{d}}+\Theta\left(R^{d-2}\right).
\end{align}
As~(\ref{volume_delta}) deals with the unscaled lattice, we now use the rescaling actions performed in Theorem 1 to move "back" to the "unscaled" version of our spherical C-Space, in order to reach the sample complexity evaluation:
\begin{align}
    \|\XL\cap \B_R\|\underset{[T2]}{=}\|\Lambda\cap\B_{R_{orig}}\|\underset{\left(\ref{volume_delta}\right)}{\leq}\frac{1}{\sqrt{\pi}d}\left(\frac{2\pi e}{d}\right)^{\frac{d}{2}}R_{orig}^d+c\left(R_{orig}^{d-2}\right) \nonumber\\
    \underset{[T2]}{=}\frac{1}{\sqrt{\pi}d}\left(\frac{R}{\beta}\right)^d\left(\frac{2\pi e}{d}\cdot f_\Lambda^2\left(d\right)\right)^{\frac{d}{2}} +  c\left(\frac{R}{\beta}\right)^{d-2}\left(f_\Lambda\left(d\right)\right)^{d-2} \nonumber\\
    \Rightarrow \|\XL\cap \B_R\| \leq \frac{1}{\sqrt{\pi}d}\left(\frac{R}{\beta}\right)^d\left(\frac{2\pi e}{d}\cdot f_\Lambda^2\left(d\right)\right)^{\frac{d}{2}} +  c\left(\frac{R}{\beta}\right)^{d-2}\left(f_\Lambda\left(d\right)\right)^{d-2},
\end{align}
with some $c>0$ from~(\ref{volume_delta}). This finishes the proof.  
\end{proof}

The following corollary leverages the last theorem and the specific structure of \Lattices to derive specific upper bounds.

\begin{cor}[$\XZ,\XD,\XA$ sample complexity]
    Fix $\beta=\beta\left(\delta,\epsilon\right)$ and let $\theta=~\theta\left(\delta,\epsilon\right):=~\frac{R}{\beta}$. Consider the configuration space  $\C=\B_R$ for $R=\sqrt{d}\beta$ or $R \geq d\beta$. Then the following bounds hold:
    \begin{enumerate}[topsep=1pt,itemsep=1ex,partopsep=1ex,parsep=1ex]
        \item 
            $|\XZ\cap\B_R| = O\left(\frac{1}{d}\left[\left(2.07\theta\right)^d+\left(\frac{d}{4}\theta\right)^\frac{d-2}{2}\right]\right)$
        \item 
            $|\XD\cap\B_R| = O\left(\frac{1}{d}\left[\left(1.46\theta\right)^d + \left(\frac{d}{8}\theta - \frac{1}{16}\theta\right)^\frac{d-2}{2}\right]\right)$
        \item 
        $|\XD\cap\B_R| = O\left(\frac{1}{d}\left[\left(1.19\theta\right)^d+\left(\frac{d}{12}\theta\right)^\frac{d-2}{2}\right]\right)$
    \end{enumerate}
\end{cor}
\begin{proof}
    First, we look at $\ZN$. From Theorem~\ref{general_sample_complexity}, we get
    \begin{align*}
        |\XZ\cap \B_R| = O\left(\frac{1}{d}\left(\theta^2\frac{2\pi e}{d}\cdot f_{\ZN}^2\left(d\right)\right)^{\frac{d}{2}} + \left(\theta\cdot f_{\ZN}\left(d\right)\right)^{d-2}\right) \\
        = O\left(\frac{1}{d}\left(\theta\sqrt{\frac{\pi e}{2}}\right)^d+\left(\theta\frac{\sqrt{d}}{2}\right)^{d-2}\right)\\
        = O\left(\frac{1}{d}\left[\left(2.07\theta\right)^d+\left(\frac{d}{4}\theta\right)^\frac{d-2}{2}\right]\right).
    \end{align*}
    Next, we look at $\DN$. From Theorem~\ref{general_sample_complexity}, we get
    \begin{align*}
        |\XD\cap \B_R| = O\left(\frac{1}{d}\left(\theta^2\frac{2\pi e}{d}\cdot f_{\DN}^2\left(d\right)\right)^{\frac{d}{2}} + \left(\theta\cdot f_{\DN}\left(d\right)\right)^{d-2}\right) \\
        = O\left(\frac{1}{d}\left(\theta^2\frac{2\pi e}{d}\cdot \frac{2d-1}{16}\right)^{\frac{d}{2}}+\left(\theta\frac{\sqrt{2d-1}}{4}\right)^{d-2}\right)\\
        =O\left(\frac{1}{d}\left(\theta^2\frac{2\pi e}{8}\cdot \frac{2d-1}{2d}\right)^{\frac{d}{2}}+\left(\theta\frac{2d-1}{16}\right)^{\frac{d-2}{2}}\right).
    \end{align*}
    But, since
    \begin{align*}
        \left(\frac{2d-1}{2d}\right)^\frac{d}{2}=\left(\left(1+\frac{\left(-1\right)}{2d}\right)^{2d}\right)^\frac{\frac{d}{2}}{2d}\overset{n\rightarrow\infty}{\longrightarrow} e^{\frac{1}{4}},
    \end{align*}
    we obtain:
    \begin{align*}
         \|\XD\cap \B_R\|=O\left(\frac{1}{d}\left(\theta\sqrt{\frac{\pi e}{4}}\right)^d+\left(\theta\frac{2d-1}{16}\right)^{\frac{d-2}{2}}\right)\\
         = O\left(\frac{1}{d}\left[\left(1.46\theta\right)^d + \left(\frac{d}{8}\theta - \frac{1}{16}\theta\right)^\frac{d-2}{2}\right]\right).
    \end{align*}
    Lastly, we look at $\AN$. From equation (7) above it can be seen that
    \[
        T^tT=G\left(EP\right)^t\left(EP\right)G^t=
        \begin{pmatrix}
            2 & 1 &  1  & \dots & 1 & -1 \\
            1 & 2  &  1 & \dots & 1 & -1 \\
            . & .  &  . & \dots & . & .  \\
            1 & 1  &  1 & \dots & 2 & -1 \\
            -1 & -1 & -1 & \dots & -1 & x
        \end{pmatrix}\in\mathbb{R}^{d\times d}, x=\frac{D-1}{D}.
    \]
    Furthermore, it can be shown that $T^tT=GG^t=Gr_\Lambda$. This means that we can use Theorem~\ref{general_sample_complexity} to approximate the number of lattice points in the embedded lattice, as they both share the gram matrix $Gr_\Lambda$---which intuitively makes sense, as they both represent the lattice (only that one of them is in a higher dimension).
    From Theorem~\ref{general_sample_complexity}, we get:
    \begin{align*}
        |\XD\cap \B_R| = O\left(\frac{1}{d}\left(\theta^2\frac{2\pi e}{d}\cdot f_{\AN}^2\left(d\right)\right)^{\frac{d}{2}} + \left(\theta\cdot f_{\AN}\left(d\right)\right)^{d-2}\right) \\
        = O\left(\frac{1}{d}\left(\theta^2\frac{2\pi e}{d}\cdot \frac{d\left(d+2\right)}{12\left(d+1\right)}\right)^{\frac{d}{2}}+\left(\theta\sqrt{\frac{d\left(d+2\right)}{12\left(d+1\right)}}\right)^{d-2}\right)\\
        =O\left(\theta^2\frac{1}{d^2}\left(\frac{2\pi e}{12}\cdot \frac{d+2}{d+1}\right)^{\frac{d}{2}}+\left(\frac{d}{12}\theta\right)^{\frac{d-2}{2}}\left(\frac{d+2}{d+1}\right)^{\frac{d-2}{2}}\right).
    \end{align*}
    But, since
    \begin{align*}
        \left(\frac{d+2}{d+1}\right)^\frac{d}{2}=\left(\left(1+\frac{1}{d+1}\right)^{d+1}\right)^\frac{\frac{d}{2}}{d+1}\overset{n\rightarrow\infty}{\longrightarrow} e^{\frac{1}{2}},\\
    \end{align*}
    and similarly for the right term, we obtain
    \begin{align*}
         |\XA\cap \B_R| =O\left(\frac{1}{d}\left(\sqrt{\theta\frac{\pi e}{6}})^d+\left(\frac{d}{12}\theta\right)^{\frac{d-2}{2}}\right)\right)\\
         = O\left(\frac{1}{d}\left[\left(1.19\theta\right)^d+\left(\frac{d}{12}\theta\right)^\frac{d-2}{2}\right]\right).
    \end{align*}
\end{proof}
    \itai{made changes here}
\subsection*{Comparing sample complexity for \Lattices}
    What is quickly clear from these results, is that in terms of sample complexity we get increasingly better evaluations going for the lattices: $\mathbb{Z}^d\rightarrow D_d^*\rightarrow A_d^*$. Both the first term and the error term of the sample complexity expression get better: 
    \begin{enumerate}
        \item The first term gets exponentially better, going from $2.07^d$ to $1.46^d$ and $1.19^d$.
        \item The error term also gets better, with its base going from $\frac{d}{4}$ to $\frac{d}{8}$ and $\frac{d}{12}$. 
    \end{enumerate}
    In both comparisons we disregarded the common $\theta$ term.
    Combining these two improvements, we see that $A_n^*$ is the superior lattice here, in terms of lattice sample density.


    Next, we show that $\XA$ leads to even better performance in terms \emph{CC-complexity}.

% We complete this section with an analysis of the CC complexity of our sample sets. 
% \begin{thm}[$\XZ,\XD,\XA$ CC complexity]
%   Consider the configuration space $\B_{r_c}$ for (rc=?). Then the following upper bounds on CC complexity hold: \kiril{Why is this missing information?}
%     \begin{enumerate}
%         \item 
%         \begin{align*}
%             \frac{\|\chi_{D_d^*,C-Space\|}}{\|\chi_{LB}\|}= ?? \\
%             \|\chi_{D_d^*,\beta-ball}\|= ??
%         \end{align*}        
%         \item 
%         \begin{align*}
%             \frac{\|\chi_{A_d^*,C-Space\|}}{\|\chi_{LB}}\|\ = ?? \\
%             \|\chi_{A_d^*,\beta-ball}\|= ??
%         \end{align*}
%     \end{enumerate}
% \end{thm}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:


==> tex/6b_Experiments_prev_version.tex <==



In this section, we will demonstrate some of the theoretical results achieved in the pape . All experiments were done with the same computer, the "Vivo Asusbook 16x" lapto . \itai{Added computer details} The first section of the paper dealt with finding the sample complexity of lattice . In the following graphs we compare the resulting theoretical sample and collision complexity with an actual count of the number of these values in a simulatio . The counting (both samples and edge lengths) was done using a BFS-like search algorithm (starting from the center of the sphere) to overcome how heavy the calculations become at higher dimensions, as our BFS-like algorithm only visits $O(d\cdot|\XL|)$ nodes.



\begin{algorithm}
\caption{Implicit-A*}\label{alg:ImpA}
\KwData{$\Lambda\in\mathbb{R}^d, R>0, p_s,p_e,\delta>0,\epsilon>0$}
\KwResult{a $(\delta,\epsilon)$-path from $p_s$ to $p_e$ on $\Lambda$}
  ${p^{data}_s \gets (Sample:p_s,IntVec:\overset{\rightarrow}{0},g:0,h:\|p_e-p_s\|)}$\;
  $O:=OPEN \gets \{p^{data}_s\}$\;
  $V:=VISITED \gets \{\overset{\rightarrow}{0}: \{p^{data}_s\}$\}\;
  $P:=PREV \gets \{p^{data}_s: null\}$\;
  $INV:=INVALID \gets \{\}$\;
  $NN\gets GetNeighbors(\Lambda,R,p_s,\delta,\epsilon)$\;
  \While{$O$ not empty}{
    $v^{min}\gets O.pop\_min()$\;
    \If{$v^{min}$ is $p_e$}{
      create path RES using PREV array P\;
      \Return RES
    }
    $\overline{NN} \gets NN$\;
    \If{$\|v^{min}-p_e\| < R$} {
      $\overline{NN} \gets \overline{NN} \cup \{p_e-v^{min}\}$\;
    }
    \For{$n$ in $\overline{NN}$} {
      \tcc{shift the neighbors to the current center}
      $n_I \gets n_I + v^{min}_I$\;
      $n \gets n + v^{min}$\;
      \If{$n$ is not goal but is INVALID}{
        \Continue
      }
      \If{n is not VALID}{
        $INV[n]=True$\;
        \Continue
      }
      \If{edge $v^{min}\rightarrow n$ is INVALID}{
        \Continue
      }
      $newG \gets v^{min}_g + n_g$\;
      $currG \gets \infty$\;
      \If{$n$ was VISITED}{
        $currG \gets V[n_I].g$\;
      }
      \If{$newG < currG$}{
        \eIf{$n$ was VISITED}{
          $n^{data} \gets V[n]$
        } {
          $n^{data} \gets (n,n_I,newG, \|n-g_e\|)$\;
          $V[n_I] \gets n^{data}$\;
        }
        $P[n^{data}]\gets v^{min}$\;
        \If{$n^{data}$ is NOT in $OPEN$}{
          $O \gets O \cup \{n^{data}\}$\;
        }
      }
    }
  }
\end{algorithm}

\subsection*{Implementation details}

All of the experiment sections require an implementation of the lattice . To do that we utilize the OMPL library---an environment developed by the Kavraki Lab~\cite{sucan2012the-open-motion-planning-library} that enables both efficient running of c++ algorithms and their testing in the OMPLapp python interfac   The lattices were using a BFS-like algorithm to actively create the sample set, allowing to get all the samples in ball / box regions, after which we run an implicit-A* run with some modification . Let us go over important implementation details in Algorithms~\ref{alg:getNN} and \ref{alg:ImpA}.
\begin{enumerate}
    \item First thing to notice is that both algs use the underlying  $\ZN$ structure that we have in every lattice, before applying the generato . Using a integer vectors to compare points instead of float vectors is quicker and more accurate.
    \item Second thing to notice is that we calculate GetNeighbors once, before the main loop, in line  . This is due to the regularity of lattice . In lines 18-19 we shift the neighbors to the current center.
    \item Last thing to notice is that we keep track of all points that were already invalidate . As each point in the lattice is visited up to $2d$ times, only checking it once saves computation time.
    \item Regarding RND sample sets, Algorithm~\ref{alg:ImpA} is well fitted to easily run them as well. The main changes that occur are: in line 6, $NN$ is calculated using some RND nearest-neighbor structure, to be later used in line 1 . After this, we need to avoid preforming the "shift" in lines 18,1 . At any place we use the integer vector to compare, we instead use a special "Vertex" structure that OMPL uses in its NN-graph . This way RND works as an "implicit-A*" for the purposes of a fair comparison.
\end{enumerate}

The integrated lattice traversal within the implicit-PRM setting will be referred to, in this section, as \emph{Lattice-PRM} (LPRM), and the the random-sample variant will be referred to as \emph{Random-PRM} (RPRM) \kiril{Unclea . Please be more precise about the algorithm her . The same applies to all the different algorithm in this section.}\itai{done + full algorithm explanations }. An important hyper-parameter involves picking the right $\delta$ value i . While the improvement over a regular grid remains, it takes less time to find a path when using the optimal clearance---optimal in the sense of runtime, not optimal path clearanc . The differences between runtimes for low and high clearance values are, as you will see, very sharp, and the right value needs to be picke . The second one is the $\epsilon$ hyper-parameter, which is less important - as we can start with "infinite" clearance to just get some solution (in practice $\epsilon=10$ is already "infinite"), and lower it if we want a better one.


The last thing to note in terms of our testing environment is that we updated the OMPLapp~\cite{sucan2012the-open-motion-planning-library} environment to be able to display paths of any $N$ disk-robots moving around.

\begin{figure}[thb]
\centering  
\includegraphics[width=0.9\columnwidth]{Images/relative_bound_quality.png}
\caption{Comparing the lattices' relative size}
\label{fig:comparative_samples}
\end{figure}

\subsection{Sample complexity}

% \begin{figure}[H]
%     \centering
%     \begin{subfigure}[b]{0.49\textwidth}
%         \includegraphics[width=\textwidth]{Images/sample_set_absolute_by_d.png}
%         \label{fig:epgt_visual1}
%         \caption{Absolute size comparison}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[b]{0.49\textwidth}
%         \includegraphics[width=\textwidth]{Images/sample_set_absolute_by_e.png}
%         \label{fig:epgt_visual1}
%         \caption{Absolute size comparison}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[b]{0.49\textwidth}
%         \includegraphics[width=\textwidth]{Images/sample_set_relative_by_d.png}
%         \label{fig:epgt_visual1}
%         \caption{Relative size comparison}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[b]{0.49\textwidth}
%         \includegraphics[width=\textwidth]{Images/sample_set_relative_by_e.png}
%         \label{fig:epgt_visual1}
%         \caption{Relative size comparison}
%     \end{subfigure}
%     \caption{Sample complexity comparison in \Lattices}
%     \label{fig:experiments2}
% \end{figure}

We start by checking the quality of our upper limits in relation to the actual count---found by using a c++ simulation of the lattices (more on its implementation in the following experiments . First off, we can return to~\Cref{fig:limit_graph_upper} and recall the theoretical comparison between the lattice sample sets sizes: as the dimension increases, $\AN$ becomes better and better (in relation to $\ZN$)---e.g. in $d=12$ it is already produces a sample set which is around $\approx 129$ times smaller. 


Second, we can look to~\Cref{fig:comparative_samples} and see that all relative quantities are close to the value  . This means that our theoretical upper bound is very close to the real on . It can also be seen that it is mostly $<1$, which makes the upper limit an actual upper limit (with the difference probably compensated by the $P_d(\cdot)$ term).


\subsection{Collision complexity}

\itai{Todo: compare the theoretical CC to the actual one, once we agree that the bounds we got are OK.}

\itai{Todo: insert sum-of-edges checking here}

\begin{figure*}[!h]
  \centering
  \subfloat[H-Map]{
    \includegraphics[width=0.3\textwidth]{Images/Hmap_basic.png}
    %\label{fig:maps_visual1}
    }
  \subfloat[Random-polygon (RP)]{
    \includegraphics[width=0.3\textwidth]{Images/rndpoly_basic.png}
    %\label{fig:maps_visual2}
    }
  \subfloat[Unique-maze (UM)]{
    \includegraphics[width=0.3\textwidth]{Images/uniquemaze_basic.png}
    %\label{fig:maps_visual3}
    }
  \
  \subfloat[Kenny (K)]{
    \includegraphics[width=0.3\textwidth]{Images/kenny_basic.png}
    %\label{fig:maps_visual4}
    }
  \caption{Four unique scenrios. The HMap is an easy map to plan i . The RndPoly map is harder to navigate than H-Map, while still having some easy solutions due to high clearance areas. The UniqueMaze map is the hardest to traverse in terms of clearance, but robots can still move independently of eachothe . Lastly, the Kenny map is the hardest map in all aspect . Not only low clearance, robots have to also move simultaneously, otherwise they would collide.}
  \label{fig:maps}
\end{figure*}

\subsection{Simulations}
% From here, the following important detail can be used in more complicated maps: when planning a multi-robot path with $n$ robots in $\mathbb{R}^{2n}$, if we maintain movement by a single robot at a time, then no matter how close the moving robot is to the obstacles - we still get the sum of clearances for the other "still" robot   This intuitively means we "inflate" the moving robot's free space, helping him move through tunnels easier.\\
% Noticing this detail, certain maps (like this H map) give rise to an easy initial clearance guess: the sum of clearance of any $n-1$ robots, given that they are still in their locatio . Very obstacle-dense maps or maps with so many robots such that they are always close to each other still pose a problem, thoug . We use this distinction in our tests to improve the test runtimes, getting an approximated clearance value (that may be needed to be adjusted . Speficially, this distinction did help me progress to testing three disks, i.e. $d=6$, with $\delta=12.5\cdot 2=25$, which will be our base for the following experiments.


\subsection*{Comparing \Lattices and random sample sets}

We continue to compare the four sample sets that we considered in the scenarios depicted in~\Cref{fig:maps}. We focus on two styles of experiments: 2-swap and 3-swa . In these, the robots have to swap places: $1\leftrightarrow2$ or $1\rightarrow2\rightarrow3\rightarrow1$ . Another aspect of the test was the comparison of $\AN$ with RND using RPRM's method of building the NN graph beforehand (unlike LPRM where we already know the neighbors . These are the rows who's NN column is marked "Yes . This was done to further compare only the \emph{structure} of the PRM graphs we recieve with both methods. 
In~\Cref{table:experiment}, specific 2,3-swap start coordinates were chosen for each ma . It can be seen that in some RND does better than $\AN$, and in some $\AN$ win . While results are summarized in the table itself, here are the main points:
\begin{enumerate}
    \item In most, the deterministic method did at least more or less as well as the probabilistic metho . Even in cases where a random set did better than $\AN$, the difference was not big.
    \item $\AN$ does not only beat $\ZN$ in all of the cases, but in a lot of them we can observe an order of magnitude improvement in runtime.
    \item We recognized a dominance of $\AN$ over RND in maps of very narrow passage . The first example can be seen in the 3-swap UniqueMaze scenario, where it is already 3 times quicker than RN . The more impressive result, though, is in the Kenny map, where RPRM struggles to even find a solutio . This map was made to force all 3 robots to move "together": none of the robots can realistically move without the others also moving, forcing a solution path which can not be broken down into single-robot-movements.
\end{enumerate}

\subsection*{Demonstrating $\AN$ on difficult scenarios}

\itai{added the demonstrative scenarios}
In this final section, we demonstrate the best performing lattice on several situations considered to be especially difficult in the multi-robot planning setting.

\begin{figure}[thb]
\centering  
\includegraphics[width=0.9\columnwidth]{Images/8-swap.png}
\caption{8-swap}
\label{fig:8-swap}
\end{figure}

The first scenario~\ref{fig:8-swap} we managed to plan is one where eight disk robots were asked to perform a swap (similar to previous 3-swaps, this is an 8-swap . An 8-swap scenario is a $d=16$ problem, which is relatively high dimensio . It took 337 seconds to finish planning this.  

\begin{figure}[thb]
\centering  
\includegraphics[width=0.9\columnwidth]{Images/slide-puzzle.png}
\caption{slide puzzle: $(1,2,3,4)\rightarrow(4,3,2,1)$}
\label{fig:slide-puzzle}
\end{figure}

The next scenario~\ref{fig:slide-puzzle} is inspired by the "16 puzzle", introducing 4 sliding pieces in a very tight environmen . Naming the piece "1" to "4" (from left to right), we want $(1,2,3,4)\rightarrow(4,3,2,1)$. The difficulty here is not the high dimension, but the extremely limited area in which the $d=8$ point robot can maneuve . This scenario took 128 minutes.



==> tex/8_Leftover_parts.tex <==
\section{LEFTOVERS}

\subsection{General lower bound}
We adapt a previous result to obtain a new lower bound on the sample complexity of \decomp sets. The bound is asymptotic with respect to the dimension, and should be contrasted with our lattice-specific bounds presented later on, which are nonasymptotic. % To simplify the analysis, for the following lemma we assume that the configuration space is a $d$-dimensional $R$-ball for some $R\in (0,\infty)$, i.e., $\C:=\B_R$.

\begin{lemma}[Verger-Gaugry's~\cite{verger2005covering} lower bound]\label{thm:sample_lower}
  Suppose that $\X$ is a  $\beta$-cover. Fix a radius $R>0$ such that  $R=\sqrt{d}\beta$ or $R\geq d\beta$, $\beta:=\beta\left(\delta,\epsilon\right)$. Then for $d>0$ large enough there exists $c>0$ such that 
    \begin{equation}\label{eq:general_LB}
        |\X| \geq   cd\left(\frac{R}{\beta}\right)^d =: n_{VG}^{\de}.
    \end{equation}
    % \triangleq \|\X_{LB}\|
\end{lemma}

\begin{proof}
Theorem 3.10 in~\cite{verger2005covering} states that if a sample set $\X^*$ is a $\frac{1}{2}$-cover for $\B_{R^*}$, where $R^*=\frac{\sqrt{d}}{2}$ or $R^*\geq\frac{d}{2}$, then there exists $c>0$ such that for $d>0$ large enough, $|\X^*|\geq cd\cdot \left(2R^*\right)^d$. Next, we use a rescaling argument to apply those findings to our setting. In particular, we wish to cover $\B_R$ with $\beta$-balls. To convert $\beta$-balls into $\frac{1}{2}$-balls we rescale $\C$ by $\frac{1}{2\beta}$, which yields a ball of radius $R^*=\frac{R}{2\beta}$. In this rescaled space, $\B_{R^*}$ is covered by $\frac{1}{2}$-balls. 

For the radius $R^*$ to fit Verger-Gaugry's requirements, we need to ensure that
\[
    \frac{R}{2\beta} = R^* = \frac{\sqrt{d}}{2},
\]
which implies that $R=\sqrt{d}\beta$, 
and similarly  %\footnote{Notice that this lower bound applies to any ball $\B_r$, as long as it is $\sqrt{d}$ times or more than $d$-times the "minimal radius" ball of $\beta$.}
$R\geq d\beta$ for the other case. Returning to Verger-Gaugry's result, we get the lower bound
\[
    |\X|=|\X^*| \geq cd\cdot \left(2R^*\right)^d = cd\cdot \left(\frac{R}{\beta}\right)^d,
\]
which concludes the proof. %\qedsymbol
\end{proof}

%\kiril{Instead of the following discussion, can you generate a plot for the two conditions $R=\delta\beta,R\geq d\cdot \beta$ in dimensions $3,6,9$, where on $x$-axis you fix $\delta$ and on the $y$-axis you plot the allowed $\eps$-range?} \kiril{Alternatively, move into appendix.} \itai{TODO: discuss this. is this part nessecary?}

%\kiril{Start of text to be commented out.}

We discuss the applicability of the above lemma in our setting and show that the requirement $R\geq d\beta$ is not overly restrictive. \kiril{Update the discussion below to $d=5$ or $6$, which is more relevant. Feel free to change the numbers, but try to stick to our setting, i.e., a ball Cspace. No need to include here all the calculations, just the outcome.}\itai{I added some computations, tell me what you think of this version} Using the requirement above, ~\Cref{lem:cover}---in which we defined $\beta(\delta,\epsilon)$, and using $d=6,R=1$, one can reach the following connection:
\begin{align*}
    \epsilon \leq \frac{1}{\sqrt{36\delta^2-1}}
\end{align*}
First, this implies a minimal clearance of ${\delta>\frac{1}{6}\approx0.17}$. Second, this shows that for low enough $\delta$ values we have an unlimited maximal $\epsilon\rightarrow\infty$ (when $\delta\downarrow0.17$). It does pose a limit on the clearance, but it still enables a good approximation in many situations. See \Cref{fig:limit_graph_lower} for the exact figure showing the relationship between $\delta$ and $\epsilon$. \itai{we may need to remove this part, as we now know that this is asymptotic. I added a note that it is asymptotic.} \kiril{let's keep it. It strengthens our lattice bounds.}\itai{done + graph}
\begin{figure}[thb]
\centering  
\includegraphics[width=0.9\columnwidth]{Images/eps_delta_lower_limit.png}
\caption{Dependence of $\epsilon$ on $\delta$ in order to get a valid lower limit (\Cref{thm:sample_lower}).}
\label{:limit_graph_lower}
\end{figure}


%  if our space's radius is $\sqrt{10}$ times bigger than a $\beta$-ball then the volume is $\sqrt{10}^{10}=10^{\frac{10}{2}}$ bigger than a $\beta$-ball. This means we expect to find about $10^5$ smaller $\beta$-balls in it. With a normal cubic $[0,1]^d$ world, we expect to find about $\frac{1}{\beta^d}=\left(\frac{1}{\beta}\right)^d=\left(\frac{1}{\beta^2}\right)^{\frac{d}{2}}$ balls. Taking the same $d=10$, we get that for our spherical space to have less $\beta$-balls than a cubic space, we will need $\frac{1}{\beta^2}\geq 10 \Rightarrow \beta \leq 0.32$. We get:
% \[
%     \beta=\delta\sqrt{\frac{\epsilon^2}{1+\epsilon^2}}\leq0.32 \iff \frac{\epsilon^2}{1+\epsilon^2}\leq \left(\frac{0.32}{\delta}\right)^2
% \]
% But notice that:
% \[
%     \frac{0.32}{\delta}<1 \iff \delta>0.32
% \]
% So for $\delta\leq 0.32$, we get $\frac{0.32}{\delta}\geq1$. But $\frac{\epsilon^2}{1+\epsilon^2}<1$ for all $\epsilon>0$, which makes the above inequality true for all $\epsilon>0$. All this is to say the following: the requirements on $\delta,\epsilon$ aren't harsh and would probably be fulfilled in most use cases, allowing us to rely on this lower bound.

We conclude this part with a comparison of the bound $n_{VG}^{\de}$ with a naive lower-bound, which asserts that the minimal number of points in a set $\X$ that is $\beta$-cover should be at least the volume of $\B_R$ divided by the volume of a $\beta$-ball, i.e., 
\begin{equation}
        |\X|\geq \frac{\partial(\B_R)}{\partial(\B_\beta)}=\frac{\partial(\B_1) R^d}{\partial(\B_ 1)\beta^d}=\left(\frac{R}{\beta}\right)^d:=n_{\text{naive}}^{\de}, 
\end{equation}
where $\partial(A)$ is the volume, or Lebesgue measure, of a set $A\subset \dR^d$. 
Notice that $n_{VG}^{\de}$ is $d$ times tighter than $n_{\text{naive}}^{\de}$, although this result is asymptotic. 


\subsection{a complicated lettice definition (not needed?)}
A lattice $\Lambda$ with a basis $E$ is defined to be:
\[
    \Lambda\triangleq\smashoperator[r]{\bigcup_{\{p=k\cdot e_i | k\in \mathbb{N},e_i\in E\}}}\{v|v\text{ is a vertex of } F_{\Lambda,p}\}
\]

\subsection{something from the lower bound section Im not sure of anymore}
with $D\subset \mathbb{R}^d$ some set. This calculation is equivalent to a sample set taken uniformly on the set $D$, spaced out by balls of radius $\epsilon>0$.  This means we can extrapolate the number of samples this lower bound would've gotten on the same $\frac{\sqrt{d}}{2}$-radius ball. We know the $[0,1]^n$-cube is of volume 1, so the new number of samples is:
\begin{align*}
    \|\chi_{new-LB}\|=\|\chi_{LB}\|*Vol(B_2(0,\frac{\sqrt{d}}{2})) \\
    =\sqrt{\frac{e}{2}}\Big(1-\frac{2\delta}{1-2\delta}\Big)^2\Big(\sqrt{\frac{d-1}{2\pi e}}\cdot \frac{1-2\delta}{\delta}\Big)^d \cdot c_d(\frac{\sqrt{d}}{2})^d \\
    =c_2c_d\cdot (d(d-1))^{\frac{n}{2}}\Big(\frac{1-2\delta}{2\delta}\Big)^d
\end{align*}
for some $c_2>0$. Comparing the two values:
\begin{align*}
    \frac{\|\chi\|}{\|\chi_{new-LB}\|} = \frac{4c_1\delta d\cdot\frac{d^{\frac{d}{2}}}{(2\delta)^d}}{kc_d\cdot (d(d-1))^{\frac{n}{2}}\Big(\frac{1-2\delta}{2\delta}\Big)^d} \\
    =\frac{c_3\delta c_d^{-1}d}{(d-1)^{\frac{n}{2}}}(1-2\delta)^d
\end{align*}
Using the same approximation for $c_d^{-1}\approx\sqrt{\pi d}(\frac{d}{2\pi e})^{\frac{d}{2}}$:
\begin{align*}
    \approx\frac{c_3\delta \sqrt{\pi d}(\frac{d}{2\pi e})^{\frac{d}{2}}d}{(d-1)^{\frac{n}{2}}}(1-2\delta)^d \\
    =c_4\delta d^{1.5}\Big(\frac{d}{d-1}\Big)^{\frac{d}{2}}\Big(\frac{1-2\delta}{\sqrt{2\pi e}}\Big)^d \\
\end{align*}
Again, using the similar calculations as the previous section, we can use $\Big(\frac{d}{d-1}\Big)^\frac{d}{2}\rightarrow \sqrt{e}$:
\begin{align*}
    \leq c_5\delta d^{1.5}\cdot\Big(\frac{1}{\sqrt{2\pi e}}\Big)^d\rightarrow 0
\end{align*}

\subsection{anstar definitions we dont need}
In general, the $A_d^*$ set , is defined through the $A_d$ set:
\begin{align}
    A_d=\{(x_i)_1^{d+1} \in \mathbb{Z}^{d+1} \mid \sum_i x_i = 0\}
\end{align}
He then continues to define the "dual" to $A_d$ as:
\begin{align}
    A_d^*=\bigcup_{i=0}^d ([i]+A_d)
\end{align}
For some vector $[i]$. 

\subsection{anstar upper bound leftovers}

Following this definition, we can use a well known result: if $T:\mathbb{R}^d\rightarrow\mathbb{R}^d$ then \\ ${Vol(T(S))=\det(T)\cdot Vol(S)}$. Let us first calculate $\det(T)$:
\begin{align}
    \det(T) = \sqrt{\det(T)\det(T)} = \sqrt{\det(T^t)\det(T)} =\sqrt{\det(T^tT)} \nonumber \\ \label{det_T}
    = \det((EPG^t)^t(EPG^t)) = \det(G(EP)^t(EP)G^t)
\end{align}
 In ~\cite{conway2013sphere}, the determinant of the lattice is defined as $\det(GG^t)$ and Conway cites it~\cite{conway2013sphere} to be $\frac{1}{d+1}$. Combine these facts with~(\ref{det_T}) and you get that $\det(T)=\sqrt{n+1}$. 


Let us use this fact to compute two things: first, let us find the size of the whole sample set. Conway~\cite{conway2013sphere} gives us the radius of the most optimal ("thinnest" in the book's terms) ball radius, which is said to be:
\begin{align}
    R=\sqrt{\frac{n(n+2)}{12(n+1)}}
\end{align}
So, let us assume we live in a cube of size $[0,w]^n$ with optimal balls of the above radius $R$. We would like the cube size to be such that if we rescale $[0,w]^n$ to $[\delta,1-\delta]^n$ we would also get $\beta$-Balls from $R$-Balls, to fit with the setting in~\cite{dayan2023near}. So:
\begin{equation}
    \begin{cases}
      wx=1-2\delta\\
      Rx=\beta
    \end{cases}
    \Rightarrow 
    \begin{cases}
         x=\frac{\beta}{R} \\
         w=\frac{(1-2\delta)R}{\beta} = \frac{1-2\delta}{\delta}\frac{R}{\alpha}
    \end{cases}
\end{equation}
So using these facts, we need a set $S\subset \mathbb{R}^d$ such that $T(S)=[0,w]^d$, getting:
\begin{align*}
    Vol(S)=\sqrt{d+1}\cdot Vol([0,w]^d)=\sqrt{d+1}\cdot(\frac{1-2\delta}{\delta}\frac{R}{\alpha})^d\\
    =\sqrt{d+1}(\frac{1-2\delta}{\delta})^d\cdot(\sqrt{\frac{d(d+2)}{12(d+1)}})^d(\frac{\sqrt{1+\epsilon^2}}{\epsilon})^d \\
    =\sqrt{d+1}(\frac{1-2\delta}{\delta})^d\cdot(\frac{d(d+2)}{12(d+1)}(1+\frac{1}{\epsilon^2}))^{\frac{d}{2}}\\
    = \sqrt{d+1}(\frac{1}{\delta} - 2)^d\cdot(\frac{d(d+2)}{12(d+1)}(1+\frac{1}{\epsilon^2}))^{\frac{d}{2}}\\
    \leq \sqrt{d+1}(\frac{1-2\delta}{\delta})^d\cdot(\frac{d(d+2)}{12(d+1)})^{\frac{d}{2}}
\end{align*}
Using similar methods, we will compute the number of samples in a ball of radius $\beta$. We want a set $\Tilde{B}\subset \mathbb{R}^d$ such that $T(\Tilde{B})=B(\delta,c)$ for some center point $c\in\mathbb{R}^d$. Remember from the last paragraph that this comes from a ball of radius $R$, so:
\begin{align*}
    \|B_\beta\cap\Lambda\|\leq \frac{Vol(B_\beta)}{\sqrt{d}}+k(\beta)^{d-2}\leq \frac{\beta^d}{\sqrt{d}c_d^{-1}}+k(\beta)^{d-2}\\
    \approx\beta^{d-2}[\frac{\beta^2}{\pi\cdot d}(\frac{d}{2\pi e})^{\frac{d}{2}} + k]\\
    \|\chi_{Ball}\|\leq Vol(\Tilde{B})=\sqrt{d+1}Vol(B(\beta,c))=\sqrt{d+1}c_dR^d\\
    =\sqrt{d+1}(\frac{d(d+2)}{12(d+1)})^{\frac{d}{2}}\frac{1}{\sqrt{\pi d}(\frac{d}{2\pi e})^{\frac{d}{2}}}\\
    =\sqrt{\frac{d+1}{\pi d}}(\frac{2\pi e \cdot (d+2)}{d+1})^{\frac{d}{2}}\rightarrow \frac{(\sqrt{\frac{2\pi e}{12}})^d}{\sqrt{\pi}}\approx\frac{1.19^d}{\sqrt{\pi}}
\end{align*}

Remembering that we want the integer vectors in this space, and that small cubes in that grid are of volume 1, we get that:
\begin{align}
    \|\chi_{A_d^*}\|\leq Vol(S)=\sqrt{d+1}(\frac{1-2\delta}{\delta})^d\cdot(\frac{d(d+2)}{12(d+1)})^{\frac{d}{2}}
\end{align}
And Comparing it now to $\|\chi_{SG^*}\|$, we get:
\begin{align*}
    \frac{\|\chi_{A_d^*}\|}{\|\chi_{SG^*}\|}\leq\frac{\sqrt{d+1}(\frac{1-2\delta}{\delta})^d\cdot(\frac{d(d+2)}{12(d+1)})^{\frac{d}{2}}}{2(\frac{1-2\delta}{\delta})^n(\frac{2d-1}{16})^{\frac{d}{2}}} \\
    =\frac{\sqrt{d+1}}{2}(\frac{16d(d+2)}{12(d+1)(2d-1)})^{\frac{d}{2}}\leq\frac{\sqrt{d+1}}{2}(\frac{16}{12\cdot2})^{\frac{d}{2}} \\
    = \frac{\sqrt{d+1}}{2}(\frac{2}{3})^{\frac{d}{2}}\rightarrow 0
\end{align*}
This is already good. It is exponentially better than the $SG^*$ set. Let us compare it to the lower bound:
\begin{align*}
    \frac{\|\chi_{A_d^*}\|}{\|\chi_{LB}\|}=\frac{\sqrt{d+1}(\frac{1-2\delta}{\delta})^d\cdot(\frac{d(d+2)}{12(d+1)})^{\frac{d}{2}}}{\sqrt{\frac{e}{2}}\Big(1-\frac{2\delta}{1-2\delta}\Big)^2\Big(\sqrt{\frac{d-1}{2\pi e}}\cdot \frac{1-2\delta}{\delta}\Big)^d} \\
    \leq \sqrt{\frac{2(d+1)}{e}}(\frac{2\pi e\cdot d(d+2)}{12(d^2-1)}))^{\frac{d}{2}} \\
    \rightarrow (\sqrt{\frac{\pi e}{6}})^d\approx1.19^d
\end{align*}
So $\|\chi_{A_d^*}\|\leq1.19^d\|\chi_{LB}\|$, compared to $1.43^d$ for the $SG^*$ set---exponentially better!
\subsection{some remains from the onion-set section}
We need to compare it to the SG*-grid coverage of the original ball. In that, we get:
\begin{align}
    \|\chi_{SG*}\|\approx2\frac{Vol(B_{\beta}(0))}{(2\frac{2}{\sqrt{2n-1}}\delta)^n}=\frac{2c_n(\frac{\sqrt{n}}{2})^n}{(2\frac{2}{\sqrt{2n-1}}\delta)^n}=2c_n(n(2n-1))^\frac{n}{2}(\frac{1}{8\delta})^n
\end{align}
In comparison:
\begin{align*}
    \frac{\|\chi\|}{\|\chi_{SG*}\|}\approx\frac{cn^{\frac{n}{2}+1}ln(n)(\frac{1}{2\delta})^n}{2c_n(n(2n-1))^\frac{n}{2}(\frac{1}{8\delta})^n}=2c\cdot c_n^{-1} \cdot nln(n)(\frac{1}{2n-1})^{\frac{n}{2}}4^n
\end{align*}
Using~\cite{tsao2020sample}, we insert an approximation for $c_n^{-1}\approx\sqrt{\pi n}(\frac{n}{2\pi e})^{\frac{n}{2}}$:
\begin{align*}
    \frac{\|\chi\|}{\|\chi_{SG*}\|}\approx 2c \sqrt{\pi n}(\frac{n}{2\pi e})^{\frac{n}{2}}\cdot nln(n)(\frac{1}{2n-1})^{\frac{n}{2}}4^n \\ 
    =2c \sqrt{\pi} n^{1.5}ln(n)(\frac{n}{2n-1})^{\frac{n}{2}}(\frac{8}{\pi e})^{\frac{n}{2}} \\
    =2c \sqrt{\pi} n^{1.5}ln(n)(\frac{2n}{2n-1})^{\frac{n}{2}}(\frac{4}{\pi e})^{\frac{n}{2}} \\
\end{align*}
On the side, we can see that:
\begin{align}
    (\frac{2n}{2n-1})^{\frac{n}{2}}=(1+\frac{1}{2n-1})^{\frac{n}{2}}=((1+\frac{1}{2n-1})^{2n-1})^{\frac{\frac{n}{2}}{2n-1}}\rightarrow e^{\frac{1}{4}}
\end{align}
So finally:
\begin{align*}
    \frac{\|\chi\|}{\|\chi_{SG*}\|}\approx 2c\sqrt{\pi}e^{\frac{1}{4}}n^{1.5}ln(n)\cdot (0.684)^n\rightarrow0
\end{align*}
So for a high enough $n\in\mathbb{N}$, we get $\|\chi\|<\|\chi_{SG*}\|$. In general, for a high enough dimension, it behaves as $\|\chi\|\approx\|\chi_{SG*}\|\cdot 0.685^n$. It can be checked that we get $\|\chi\|<\|\chi_{SG*}\|$ starting at $n=c\cdot 19$: the $c>0$ is not specified in any of the referenced material, but assuming $c>1$, this makes the onion set impractical for motion planning problems, as we rarely reach robots with $n\geq 19$.

\subsection{ONION set leftovers: taken out of the paper for now}

\kiril{The following hasn't been defined. Why it's here?}
\begin{align*}
    \frac{\|\chi_{Onion, C-Space}\|}{\|\chi_{LB}\|} = O(\ln{d})
\end{align*}
\subsection*{Complexity of sample sizes: the non-constructive "Onion" set}

To show what's theoretically possible, using a non-constructive method, we'll be using in this section a covering set from a paper in~\cite{verger2005covering} that used an "onion" like construction to cover $\B_{\beta}(0)\subset\mathbb{R}^d$ (instead of a cube). Intuitively, this is what he does:
\begin{enumerate}
    \item Cover a sphere $S_{R}(0)$ for some $R>0$, using balls of radius $r=\frac{1}{2}$. 
    \item Show that this collection of spheres actually covers an annulus from $R$ to $R-\frac{1}{2R}$.
    \item Recursively cover smaller and smaller annuluses, until the smaller radius is less than $\frac{1}{2}$, allowing you to cover it with one extra ball.
\end{enumerate}
It can be noted that (1) is done using probabilistic methods, making the whole set non-constructive.
Using this method, he manages to cover a ball of radius $R\geq \frac{\sqrt{d}}{2}$ with $n$ balls of radius \(\frac{1}{2}\), with:
\[
    n \leq c\cdot dln(d)(2R)^d
\]
We need to cover the spherical C-Space $\B_\frac{\sqrt{d}}{2}$ with balls of radius $\beta$, so let us resize the sphere: turn balls of radius $\beta$ into balls of radius $\frac{1}{2}$, so resizing the whole space by a factor of $\frac{1}{2\beta}$. This turns the ball of radius $\frac{\sqrt{d}}{2}$ to a ball of radius $\frac{\sqrt{d}}{4\beta}$.


Our problem is, then: cover a ball of radius $\beta=\frac{\sqrt{d}}{4\delta}$ with balls of radius $\frac{1}{2}$, which falls under~\cite{verger2005covering} if:
\[
    \frac{\sqrt{d}}{4\beta} \geq \frac{\sqrt{d}}{2} \Rightarrow \beta \leq \frac{1}{2}
\]
Which is reasonable. This gives us:
\begin{align}
    \|\chi\|\leq cdln(d)(2\frac{\sqrt{d}}{4\beta})^d
\end{align}
Comparing it to the same lower bound all other lattices were compared to, we get:
\begin{align*}
    \frac{\|\chi_{Onion, C-Space}\|}{\|\chi_{LB}\|} \leq \frac{cdln(d)(2\frac{\sqrt{d}}{4\beta})^d}{k\cdot d (2\frac{\sqrt{d}}{4\beta})^d} =\frac{c}{d}\ln{d}
    \Rightarrow \frac{\|\chi_{Onion, C-Space}\|}{\|\chi_{LB}\|} = O(\ln{d})
\end{align*}
This means that this semi-random set achieves a covering that is only $O(\ln{d})$ times above the lower bound!

\subsection{calcing anstar $\rho$}

 From pages LXII and 10 of Conway~\cite{conway2013sphere}, we know 
    \[
        \rho = (\delta\sqrt{\det{\Lambda}})^{\frac{1}{d}}
    \]
    where $\delta$ is a parameter given in page 115 which is independent of choice of basis. The only thing left to calculate, then, is $\det{\Lambda}=det(G_\Lambda G_\Lambda^t)$. Let us calculate it:
    \begin{align*}
        \det{\Lambda}&=det(G_\Lambda G_\Lambda^t)\\
        &=\det\begin{pmatrix}
            1 & -1 &  0  & \dots & 0 & 0 & 0 \\
            0 & 1  &  -1 & \dots & 0 & 0 & 0 \\
            . & .  &  . & \dots & . & .  & .\\
            0 & 0  &  0 & \dots & 1 & -1 & 0\\
            \frac{-d}{d+1} & \frac{1}{d+1} & \frac{1}{d+1} & \dots & \frac{1}{d+1} & \frac{1}{d+1} & \frac{1}{d+1}
        \end{pmatrix}
        \begin{pmatrix}
            1 & 0 & \dots & 0 & 0 & \frac{-d}{d+1} \\
            -1 & 1 & \dots & 0 & 0 & \frac{1}{d+1} \\
            0 & -1 & \dots & 0 & 0 & \frac{1}{d+1} \\
            . & . & \dots & . & .  & .\\
            0 & 0 & \dots & 0 & -1 & \frac{1}{d+1}\\
            0 & 0 & \dots & 0 & 0 & \frac{1}{d+1}
        \end{pmatrix}\\
        &=\det\begin{pmatrix}
            2 & -1 &  0  & 0 & 0 &\dots & 0 & 0 & -1\\
            -1 & 2  &  -1 & 0 & 0 &\dots & 0 & 0 & 0\\
            0 & -1  &  2 & -1 & 0 & \dots & 0 & 0 & 0\\
            . & .  &  . & . & . & \dots & . & . & .\\
            0 & 0  &  0 & 0 & 0 & \dots & -1 & 2 & 0\\
            -1 & 0  &  0 & 0 & 0 &\dots & 0 & 0 & \frac{d}{d+1}\\
        \end{pmatrix},\\
    \end{align*}
    now add all $d-1$ rows to the last row:
    \begin{align*}
        &=\det\begin{pmatrix}
            2 & -1 &  0  & 0 & 0 &\dots & 0 & 0 & -1\\
            -1 & 2  &  -1 & 0 & 0 &\dots & 0 & 0 & 0\\
            0 & -1  &  2 & -1 & 0 & \dots & 0 & 0 & 0\\
            . & .  &  . & . & . & \dots & . & . & .\\
            0 & 0  &  0 & 0 & 0 & \dots & -1 & 2 & 0\\
            0 & 0  &  0 & 0 & 0 &\dots & 0 & 1 & \frac{d}{d+1}-1\\
        \end{pmatrix}\\
        &=\det\begin{pmatrix}
            2 & -1 &  0  & 0 & 0 &\dots & 0 & 0 & -1\\
            0 & 1.5  &  -1 & 0 & 0 &\dots & 0 & 0 & 0.5\\
            0 & -1  &  2 & -1 & 0 & \dots & 0 & 0 & 0\\
            . & .  &  . & . & . & \dots & . & . & .\\
            0 & 0  &  0 & 0 & 0 & \dots & -1 & 2 & 0\\
            0 & 0  &  0 & 0 & 0 &\dots & 0 & 1 & \frac{d}{d+1}-1\\
        \end{pmatrix}\\
        &=\frac{1}{2}\det\begin{pmatrix}
            2 & -1 &  0  & 0 & 0 &\dots & 0 & 0 & -1\\
            0 & 3  &  -2 & 0 & 0 &\dots & 0 & 0 & -1\\
            0 & -1  &  2 & -1 & 0 & \dots & 0 & 0 & 0\\
            . & .  &  . & . & . & \dots & . & . & .\\
            0 & 0  &  0 & 0 & 0 & \dots & -1 & 2 & 0\\
            0 & 0  &  0 & 0 & 0 &\dots & 0 & 1 & \frac{d}{d+1}-1\\
        \end{pmatrix}\\
            &=\frac{1}{2}\det\begin{pmatrix}
            2 & -1 &  0  & 0 & 0 &\dots & 0 & 0 & -1\\
            0 & 3  &  -2 & 0 & 0 &\dots & 0 & 0 & -1\\
            0 & 0  &  \frac{4}{3} & -1 & 0 & \dots & 0 & 0 & \frac{-1}{3}\\
            . & .  &  . & . & . & \dots & . & . & .\\
            0 & 0  &  0 & 0 & 0 & \dots & -1 & 2 & 0\\
            0 & 0  &  0 & 0 & 0 &\dots & 0 & 1 & \frac{d}{d+1}-1\\
        \end{pmatrix}.
    \end{align*}
    we keep going like this until the last row, getting
    \begin{align*}
        &=\frac{1}{(d-1)!}\det\begin{pmatrix}
            2 & -1 &  0  & 0 & 0 &\dots & 0 & 0 & -1\\
            0 & 3  &  -2 & 0 & 0 &\dots & 0 & 0 & -1\\
            0 & 0  &  4 & -3 & 0 & \dots & 0 & 0 & -1\\
            . & .  &  . & . & . & \dots & . & . & .\\
            0 & 0  &  0 & 0 & 0 & \dots & 0 & d & -1\\
            0 & 0  &  0 & 0 & 0 &\dots & 0 & 1 & \frac{d}{d+1}-1\\
        \end{pmatrix}\\
        &=\frac{1}{(d-1)!}\det\begin{pmatrix}
            2 & -1 &  0  & 0 & 0 &\dots & 0 & 0 & -1\\
            0 & 3  &  -2 & 0 & 0 &\dots & 0 & 0 & -1\\
            0 & 0  &  4 & -3 & 0 & \dots & 0 & 0 & -1\\
            . & .  &  . & . & . & \dots & . & . & .\\
            0 & 0  &  0 & 0 & 0 & \dots & 0 & d & -1\\
            0 & 0  &  0 & 0 & 0 &\dots & 0 & 0 & \frac{d}{d+1}-1+\frac{1}{d}\\
        \end{pmatrix}\\
        &=\frac{1}{(d-1)!}\cdot d!(\frac{1}{d(d+1)})
        =\frac{1}{d+1}.
    \end{align*}

    The following short lemma will help us get the diameter.
\begin{lemma}\label{lemma:diameter}
    Let $\{e_i\}$ be vectors such that $\angle\left(e_i,e_j\right)\leq \frac{\pi}{2}$ for all $i\neq j$. Then, the diameter of the FR created by these vectors is $\D=\|\sum_i e_i\|$.
\end{lemma}
\begin{proof}
    \begin{align*}
        \|e_i+e_j\|^2&= \|e_i\|^2+\|e_j\|^2+2\langle e_i,e_j \rangle \\
        &= \|e_i\|^2+\|e_j\|^2+2\cos{\left(\angle\left(e_i,e_j\right)\right)}\|e_i\|\|e_j\|,
    \end{align*}
    and if $\angle\left(e_i,e_j\right)\leq \frac{\pi}{2}$ then $\cos{\left(\angle\left(e_i,e_j\right)\right)}\geq 0$, so \(\|e_i+e_j\|^2 \geq \|e_i\|^2\), giving us \(\|e_i+e_j\| \geq \|e_i\|\).
    
    
    Overall, this means that we can keep adding base FR elements such that the norm keeps getting larger, until we can't add more elements. At the end, the distance between $v=0,w=\sum_i e_i$ is the largest it can be. Seeing as how the vertices of the FR are also its extreme points, we can not make it larger, meaning we found the diameter.
\subsection{LEFTOVERS from the old collision complexity proof}
We start with introducing a few basic definitions that would be used throughout this section. First, we define a \emph{fundamental region} (FR) of a lattice, which is the closed set contained inside the linear combination of that lattice's basis vectors. The geometric shape of a given FR can be viewed as ``lattice tile'', as interior-disjoint translations of it can be used to cover the space. \kiril{Are the following definitions taken from somewhere or brand new? If the former then a citation would be good.}

%This creates something that can be viewed as the "lattice tile" (see Figure~\ref{fig:reflection)), which is because the union of all the FRs covers (tile) the space. 

 \begin{figure}
    \centering
    \includegraphics[width=0.66\linewidth]{Images/FR_2D.png}
    \caption{Examples of FR tiles in $d=2$. \kiril{Explain what we see here. E.g., what are the basis and FRs?} }
    \label{fig:reflection}
\end{figure}

%From this illustration, it can be also seen that FRs are not unique, some even having a completely different basis.

% Also called a \emph{Parallelotope} sometimes. 
\begin{definition}[Fundamental region]
    For a given lattice $\Lambda$ with a basis ${E_\Lambda=\{e_i\in \dR^d\}_{i=1}^m}$ (where $m\leq d$), and a point $p\in \dR^d$, the FR is defined as 
    \begin{align*}
        F_{\Lambda,p}:=\left\{p+\sum_{i=1}^m a_i e_i\middle|\,a\in[0,1]^m\right\}. 
    \end{align*}
    The center of $F_{\Lambda,p}$ is defined to be \[c_{\Lambda,p}=p+\frac{1}{2^{m}}\sum_{a\in \{0,1\}^m}\sum_{i=1}^ma_ie_i.\]
\end{definition}
\kiril{Way may consider removing $p$ from the definition of the FR.}
We mention that the geometric shape of a FR can is not unique, which follows from non-uniqueness of the lattice basis (see Figure~\ref{fig:reflection}). 

\kiril{Ideally, figures should be saved as pdfs (or other vector formats). I usually used \url{http://ipe.otfried.org/}.}.


% A for a given FR, its center is the average of all binary linear combinations of basis vectors, which means $2^{|E_\Lambda|}$ of them. \kiril{add it to the FR figure}
% \begin{definition}[FR center]\label{def:lattice_center}
%     Given a lattice $\Lambda$ with basis ${E_\Lambda=\{e_i\in \dR^d\}_{i=1}^m}$, the center of the FR $F_{\Lambda,p}$ in relation to some point $p\in \mathbb{R}^d$, is
% \end{definition}

\begin{lemma}\label{Lattice-properties}
    An FR center \(c_{\Lambda,p}\) for a  lattice \(\Lambda\) with basis ${E_\Lambda=\{e_i\in \dR^d\}_{i=1}^m}$ (where $m\leq d$) has the following properties: 
    \begin{enumerate}
        \item \(c_{\Lambda,p}=p+\frac{\sum_{i=1}^m e_i}{2}\), i.e., the center of the FR is the average of the base vectors; \kiril{Is average the right word here if we divide by $2$?}
        \item \(\{c_{\Lambda,p_i}|p_i\in\Lambda\}=\Lambda+c_{\Lambda,o}\), i.e., the collection of centers of FR regions whose point offset is a lattice point, is equal to the lattice translated with the center of the FR $F_{\Lambda,o}$, where $o$ is the origin of $\dR^d$.
    \end{enumerate}
\end{lemma}
\begin{proof}
    For the first property, we rely on the definition of $c_{\Lambda,p}$ and expand the summation expression within it. In particular, we decompose it by individually choosing the $a_i$ values, and separating the inner sum according to the dependencies on $a_i$'s. That is,
%    use a combinatorial argument. Fix a value for $a_1$. If the rest of the $a_j$ values for $j\neq i$  are chosen, then we get two "copies" of the series: one where $a_i=0$ and one where $a_i=1$. So, the relative weight of each vector is $\frac{1}{2}$. More formally, notice that
 \kiril{Please check that it makes sense.}    \begin{align*}
  \sum_{a\in \{0,1\}^m}\sum_{i=1}^ma_ie_i &= \sum_{a_1=0}^1\ldots \sum_{a_m=0}^1\sum_{i=1}^ma_ie_i \\ &=
\sum_{a_1=0}^1\ldots \sum_{a_m=0}^1a_1e_1+\sum_{a_1=0}^1\ldots \sum_{a_m=0}^1\sum_{i=\bm{2}}^ma_ie_i \\ &=
\sum_{a_{\bm{2}}=0}^1\ldots \sum_{a_m=0}^1e_1+\sum_{a_1=0}^1\ldots \sum_{a_m=0}^1\sum_{i=\bm{2}}^ma_ie_i                             \\
                                      &=
2^{m-1}e_1+2\sum_{a_{\bm{2}}=0}^1\ldots \sum_{a_m=0}^1\sum_{i=\bm{2}}^ma_ie_i                             \\
                                        &=
2^{m-1}e_1+2\cdot 2^{m-2}e_2+ 2\cdot 2\sum_{a_{\bm{3}}=0}^1\ldots \sum_{a_m=0}^1\sum_{i=\bm{3}}^ma_ie_i                             \\  & = \ldots = 2^{m-1}\sum_{i=1}^m e_i. 
    \end{align*}
    Thus, $c_{\Lambda,p}=p+\frac{\sum_{i=1}^m e_i}{2}$.

    Now consider the second property. From the previous paragraph it follows that $c_{\Lambda,o}=\frac{\sum_ie_i}{2}$. For some $p_i\in \Lambda$ it holds that
    \[c_{\Lambda,p_i}=p_i+\frac{\sum_{i=1}^m e_i}{2}= p_i+o+\frac{\sum_{i=1}^m e_i}{2}=p_i + c_{\Lambda,o},\]
    which completes the proof. 
\end{proof}

\begin{lemma}\label{fr_shifted_sum} Consider an FR $F:=F_{\Lambda,p}$ for a lattice $\Lambda$. Then, 
    \[
        I_{F,p} = I_{F,o} - |P_F|\cdot \|c_{\Lambda,p}\|^2.
    \]
\kiril{The notations here are still rather confusing. In the equation, is $p$ the same as in $F_{\Lambda,p}$, or should be $p'$? There's also ambiguity with respect to $c_{\Lambda,p}$ since it doesn't explicitly reflect a specific FR. I suggest to change it to $c(F_{\Lambda,p})$ for clarity.}
\end{lemma}
\begin{proof}
  The statement follows from expanding the definition of $I_{F,p}$:
    \begin{align}
        I_{F,p} &= \sum_{x\in P_F} \|x-c_{\Lambda,p}\|^2 = \sum_{x\in P_F} \sum_{j=1}^d \left(x(j)-c_{\Lambda,p}(j)\right)^2 \nonumber\\
        &= \sum_{x\in P_F} \sum_{j=1}^d \left(x(j)^2-2x(j)c_{\Lambda,p}(j)+c_{\Lambda,p}(j)^2\right) \nonumber\\
        &=\sum_{x\in P_F} \sum_{j=1}^d x(j)^2 + \sum_{x\in P_F} \sum_{j=1}^d c_{\Lambda,p}(j)^2 - 2\sum_{x\in P_F} \sum_{j=1}^d x(j)c_{\Lambda,p}(j) \nonumber\\
        &= I_{F,o} + |P_F|\cdot\|c_{\Lambda,p}\|^2 - 2 \sum_{j=1}^d \sum_{x\in P_F} x(j)c_{\Lambda,p}(j) \nonumber \\
        &= I_{F,o} + |P_F|\cdot\|c_{\Lambda,p}\|^2 - 2 \sum_{j=1}^d c_{\Lambda,p}(j) \sum_{x\in P_F} x(j) \nonumber \\
        &= I_{F,o} + |P_F|\cdot\|c_{\Lambda,p}\|^2 - 2 \sum_{j=1}^d c_{\Lambda,p}(j) \underbrace{\left(\sum_{x\in P_F} \left(x(j) - c_{\Lambda,p}(j)\right)+\sum_{x\in P_F} c_{\Lambda,p}(j)\right)}_\text{(*)}. \label{eq:IFo}
    \end{align}
    Next, we show that the expression in ($*$) is equal to $|P_F|c_{\Lambda,p}(j)$. In particular, we rely on the fact that for any given $x\in P_F$ it holds that $x=p+\sum_1^m a_ie_i$ for some $a\in\{0,1\}^m$ (and vice versa).
    Thus, 
    \begin{align*}     c_{\Lambda,p}&=p+\frac{1}{2^{m}}\sum_{a\in \{0,1\}^m}\sum_{j=1}^ma_ie_i \\ & =\frac{1}{2^m}\sum_{a\in \{0,1\}^m}\left(p+\sum_{j=1}^m a_ie_i\right)\\
      & =\frac{1}{2^m}\sum_{x\in P_F}x.%\\
%     &=\frac{1}{2^{|E_\Lambda|}}\sum_{j=1}^{|E_\Lambda|} x(j),\\
%        &\Rightarrow 2^{|E_\Lambda|}c_{\Lambda,p}=\sum_{j=1}^{|E_\Lambda|} x(j)\Rightarrow 0=\sum_{j=1}^{|E_\Lambda|} \left(x(j)-c_{\Lambda,p}\right),
    \end{align*}
    \kiril{I fixed some equations, which I believe were incorrect. Please check me.}
    Hence, $c_{\Lambda,p}(j)=\frac{1}{2^m} \sum_{x\in P_F}x(j)$, for $1\leq j\leq d$, 
    which implies that the vertices of the FR are symmetric around the center, intuitively speaking. From here we obtain
    \[(*)=\sum_{x\in P_F} c_{\Lambda,p}(j)=|P_F|c_{\Lambda,p}(j),\]
which we plug into \eqref{eq:IFo} to yield
    \begin{align*}
        I_{F,p}&=  I_{F,o} + |P_F|\|c_{\Lambda,p}\|^2 - 2 |P_F|\sum_{j=1}^d c_{\Lambda,p}(j)^2 \\
        &= I_{F,o} + |P_F|\|c_{\Lambda,p}\|^2 - 2|P_F|\|c_{\Lambda,p}\|^2 = I_{F,o} - |P_F|\|c_{\Lambda,p}\|^2.
    \end{align*}
\end{proof}

Notice that the value of $I_{F,p}$ is independent  of the particular point $p$: this notation talks about the sum-of-edges distance from the center of some cell that is located at an unknown location. The $p$ just denotes where the corner of the cell is, and this property \emph{does not effect} the distance from the center. \kiril{I still don't see why this is true. More care should be taken where explaining this claim.} \itai{I tried a different explanation. let's discuss it if you think it's not enough.} \kiril{Also, we already have $I_\Lambda(r)$, which looks similar.} \kiril{I want to revisit this statement after we improve the notation.} Hence, from now we denote $I_{\Lambda}:=I_{F,p}$ for some FR $F$ and point $p$. Thus, we can simplify the previous lemma statement to 
%\equiv CONST\) for any $F$ you choose, so we will just call it \(I_{\Lambda}\) from now on. Also, in our case since we are using a lattice, it has $|P_F|=2^d$ vertices, so we will just use that from now on. So we rephrase our lemma to appear as such:
\begin{align}
            I_{F,o} = I_\Lambda + 2^d\cdot \|p\|^2,
\end{align}
which holds in our case since  $|P_F|=2^d$ for our three lattices. $\ZN,\DN$ have $d$-dim bases in $\mathbb{R}^d$ and $\AN$ has a $d$-dim base in $\mathbb{R}^{d+1}$.
% \begin{lemma}
%     Let \(D_{i,r}\) be the $D_i$ such that \(\{p_i\in D_i\}\cap \B_r(0)\neq \phi\) (all the cells that contribute a vertex in the ball). Then:
%     \[
%         \lim_{n\rightarrow \infty}I(r)=\lim_{n\rightarrow \infty}{\frac{1}{N}\sum_{D_{i,r}} I_{0,D_i}}
%     \]
% \end{lemma}
% \begin{proof}
%     I know that for most of the ball, each vertex is counted N times (once for each neighbor). The trick here is to show that for the vertices that are on the edge of the ball, that are covered less than N times, the contribution to the sum goes to 0 asymptotically.
% \end{proof}
We now move to first major contribution of this section, which is a general upper-bound on collision complexity.
\begin{thm}[Collision-complexity upper bound]\label{complexity_upper_bound}
    Let $\Lambda$ be a lattice and let $F$ be some FR for the basic $E_\Lambda$. Denote by $\D$ the diameter of $F$, which is the diameter of the smallest sphere that contains $F$. Let $\rho$ be the inradius of $F$, which is the radius of the biggest  sphere that fits within $F$.
For any $r>0$ it holds that
\begin{align*}
        I\left(r\right) \leq \frac{1}{4}\left(\sum_{e\in E_\Lambda}\|e\|^2\right) \btheta^{d-1}\left(\frac{\btheta}{\rho d}+1\right)\left(\frac{\vol(\B_1)}{\sqrt{d}}\btheta+ \alpha\right), 
    \end{align*}
    where $\alpha$ is some positive constant, and
    \[
        \btheta:=\frac{r+\D-\rho}{\beta}f_\Lambda.
    \]
\kiril{We already used $\btheta$ for a different purpose.}\kiril{It would be good to visualize this theorem.} \kiril{Remove the parts related to rescaling.}
    %Then for some radius $r>0$, if we use $\theta\left(\beta,R\right):=\frac{R}{\beta}$ from corollary~\ref{cor:specific_sample_complexity} and define the rescaled radius to be
    %\[
    %    \btheta=\theta\left(\beta,r+\D-\rho\right)f_\Lambda,
    %\]
    %we get
    % \[
    %     g:=\frac{r+D-\rho}{\beta}f_\Lambda
    % \]
    % \begin{align*}
    %     g(r)&:=\frac{r-\rho}{\beta}f_\Lambda,\\
    %     % a_n(r)&:=\frac{I_\Lambda}{2^n}(\frac{Vol(\B_1)}{\sqrt{n}}g(r)^2 + k_1),
    % \end{align*}
    % we get
\end{thm}
\begin{proof}
    %First note that for now, we will use the unscaled space. Later, we will be using $\btheta$ instead of just $r+\D-\rho$, because it performs a rescaling. This is done to enable us to use the lattice point bound in equation (9) above.\kiril{Those statements are quite vague and I don't follow them.}
  We start by showing that
    \begin{align}
        I\left(r\right)\leq \sum_{i=1}^{[\frac{r+\D}{\rho}]-1} \frac{I_\Lambda}{2^d}(r+\D-i\rho)^{d-2}\left(\frac{ \vol\left(\B_1\right)}{2^d}\left(r+\D-i\rho\right)^2+\alpha\right).
    \end{align}
    Let
    \begin{align*}
        J\left(r\right):=\frac{1}{2^d}\smashoperator[r]{\sum_{F\in \F_r}} I_{F,o},
    \end{align*}
     be the partial sum-of-squares approximation, only using FRs fully contained in the $r$-ball (denoted by the set $\F_r$) \kiril{This definition is vague, and should be defined more formally.}).
     For a given FR $F\in \F_r$, denote by $c_F$ its center.
    %$$C:=\{c_F| F\subset \B_r\}.$$
     Then using \Cref{fr_shifted_sum} we obtain   \begin{align*}
        J\left(r\right)&= \frac{1}{2^d}\smashoperator[r]{\sum_{F\in \F_r}} I_{F,o} \underset{[L\ref{fr_shifted_sum}]}{=} \frac{1}{2^d}\smashoperator[r]{\sum_{F\in \F_r}} \left(I_\Lambda + 2^d\|c_F\|^2\right)\\
        &=\smashoperator[r]{\sum_{F\in \F_r}}\frac{I_\Lambda}{2^d} + \smashoperator[r]{\sum_{F\in \F_r}}\|c_F\|^2. %\leq \frac{I_\Lambda}{2^d}|B_{r-\rho}\cap\Lambda|+\smashoperator[r]{\sum_{F\in \F_r}}\|c_F\|^2. 
    \end{align*}
   Next, we observe that $|\F_r|\leq |\B_{r-\rho}\cap \Lambda|$: every FR fully included  which  follows from \kiril{be more explicit here w.r.t to the definition of $I_\Lambda$ and why this property follows. }. We also notice that $\sum_{F\in \F_r}\|c_F\|^2\leq I(r-\rho)$, which follows the second property in~\Cref{Lattice-properties}. In particular, \kiril{be more formal and include all the necessary notations and definitions.} the lemma shows that the collection of centers of is itself is a "smaller copy" of the main lattice. More than that, from the symmetry of the FR we can say that the insphere which defines the inradius is centered around the centroid (\itai{I hope this is right, otherwise I need to make some changes to this lemma}). Seeing as the insphere is included in the FR, and that we picked only the FRs that are included in the ball, we can safely reduce the radius of the ball by the inradius and still have all the centroids we started with. Therefor, using the bound on $|\B_r\cap\Lambda|$ we got at theorem~\ref{general_sample_complexity}, we get
    \begin{align}
        &\overset{\leq}{[L\ref{Lattice-properties}]} \frac{I_\Lambda}{2^d}\cdot|B_{r-\rho}\cap\Lambda| + I\left(r-\rho\right) \nonumber\\
        &\overset{\leq}{[T\ref{general_sample_complexity}]} \frac{I_\Lambda}{2^d}\cdot\left(\frac{Vol\left(\B_{r-\rho}\right)}{\sqrt{d}}+a\left(r-\rho\right)^{d-2}\right) + I\left(r-\rho\right) \nonumber\\
        &=\frac{I_\Lambda}{2^d}\cdot\left(\frac{Vol\left(\B_1\right)}{\sqrt{d}}\cdot \left(r-\rho\right)^d+a\left(r-\rho\right)^{d-2}\right) + I\left(r-\rho\right)\nonumber\\
        &=\frac{I_\Lambda}{2^d}\left(\frac{Vol\left(\B_1\right)}{\sqrt{d}}\left(r-\rho\right)^2 + a\right)\left(r-\rho\right)^{d-2} + I\left(r-\rho\right) \nonumber\\
        &=b_d\left(r\right)\left(r-\rho\right)^{d-2} + I\left(r-\rho\right)
    \end{align}
    For $b_d\left(r\right):=\frac{I_\Lambda}{2^d}\left(\frac{Vol\left(\B_1\right)}{\sqrt{d}}\left(r-\rho\right)^2 + a\right)$. Notice that $J\left(r\right)$ counts some edges too few times: edges near the border of the sphere may appear in less than $2^d$ neighboring cells, due to some cells not being included in $J\left(r\right)$, so dividing by $2^d$ lowers their contribution too much. To solve this, we will notice that for a given FR we can take the diameter $\D$ and expand $B_r$ with it. Doing this, every relevant point of $B_r$ will now contain all $2^d$ neighboring cells in the $B_{r+\D}$ ball. We do have extra points now, but the normalizer $\frac{1}{2^d}$ makes sure their contribution decays to 0. We get
    \[
        I\left(r\right)\leq J\left(r+\D\right),
    \]
    and overall
    \begin{align*}
        I\left(r\right) &\leq J\left(r+\D\right) \overset{\left(13\right)}{\leq} b_d\left(r+\D\right)\left(r+\D-\rho\right)^{d-2} + I\left(r+\D-\rho\right)\\
        &\leq b_d\left(r+\D\right)\left(r+\D-\rho\right)^{d-2} + b_d\left(r+\D-\rho\right)\left(r+\D-2\rho\right)^{d-2} + I\left(r-2\rho\right) \\
        &\leq \dots,
    \end{align*}
    which we continue until
    \[
        r+\D-m\rho < \rho \Rightarrow \frac{r+\D}{\rho} - 1 < m.
    \]
    This means we stop at \(m=[\frac{r+D}{\rho}]-1\), getting
    \begin{align*}
        I\left(r\right) &\leq \sum_{i=1}^{[\frac{r+\D}{\rho}]-1} b_d\left(r+\D-\left(i-1\right)\rho\right)\left(r+\D-i\rho\right)^{d-2}\\
        &= \sum_{i=1}^{[\frac{r+\D}{\rho}]-1} \frac{I_\Lambda}{2^d}\left(\frac{Vol\left(\B_1\right)}{\sqrt{d}}\left(r+\D-i\rho\right)^2 + k_1\right)\left(r+\D-i\rho\right)^{d-2}\\
        &=\sum_{i=1}^{[\frac{r+\D}{\rho}]-1} \left(\frac{I_\Lambda Vol\left(\B_1\right)}{2^d\sqrt{d}}\left(r+\D-i\rho\right)^d+k_1\frac{I_\Lambda}{2^d}\left(r+\D-i\rho\right)^{d-2}\right)\\
    \end{align*}
    which is because the last $I\left(r+\D-m\rho\right)=0$, due to capturing either nothing or a single point. 
    
    
    Now that we finished our base upper bound, we can now finish the theorem by further developing it. Using $k=[\frac{r+\D}{\rho}]-1$, and utilizing the known comparison between sums and integrals, we develop the following
    % Notice that $J(r)$ counts some edges too few times: edges near the border of the sphere may appear in less than $2^d$ neighboring cells, so dividing by $2^d$ lowers their contribution too much. To solve this, we will notice that for a FR we can take the diameter $D:=\text{Diam}(FR)$ and expand $B_r$ with it. Doing this, every relevant point of $B_r$ will now contain all $2^d$ neighboring cells in the $B_{r+D}$ ball. We do have extra points now, but the normalizer $\frac{1}{2^d}$ makes sure their contribution decays to 0. We get
    % \[
    %     I(r)\leq J(r+D)
    % \]
    % Which is because v is the longest vector out of all the others in the cell (as he is a sum of all of them, and they are positive (<- show this)). Due to this, the larger radius now contains all cells we didn't count before with a few more - but they are counted less, as they are weighted with $\frac{1}{2^n}$.
    \begin{align}
        &A\sum_1^k \left(r+\D-i\cdot \rho\right)^{d-B} \nonumber\\
        &\leq A\Big[\left(r+\D - 1\cdot \rho\right)^{d-B} + \int_1^k \left(r+\D-x\cdot \rho\right)^{d-B} dx\Big] \nonumber\\
        &= A\Big[\left(r+\D-\rho\right)^{d-B} + [\frac{\left(r+\D-k\cdot \rho\right)^{d-B+1}}{-\rho\left(d-B+1\right)}-\frac{\left(r+\D-\rho\right)^{d-B+1}}{-\rho\left(d-B+1\right)}]\Big] \nonumber\\
        &=A\Big[\left(r+\D-\rho\right)^{d-B} + \frac{1}{\rho\left(d-B+1\right)}[\left(r+\D-\rho\right)^{d-B+1} - \left(r+\D-k\cdot \rho\right)^{d-B+1}]\Big].
        %=_{(2)} (r+\|v\|)^n + \frac{1}{\rho(n+1)}[(r+\|v\|)^{n+1} -((n+1)k\rho(r+\|v\|)^n+O(smaller?)+(r+\|v\|)^{n+1})] \\
    \end{align}
    We also know that 
    % \begin{align*}
    %         k=[\frac{r+\|v\|}{\rho}]-1\geq \frac{r+\|v\|}{\rho}-2 \\
    %         \Rightarrow k\rho \geq r+\|v\|-2\rho \\
    %         \Rightarrow 1-k\rho \leq 1 - (r+\|v\|) + 2\rho
    % \end{align*}
    \begin{align*}
            k&=[\frac{r+\D}{\rho}]-1\leq \frac{r+\D}{\rho}-1 \\
            &\Rightarrow k\rho \leq r+\D-\rho \Rightarrow -k\rho \geq -\left(r+\D\right)+\rho \\
            &\Rightarrow r+\D-k\rho \geq \rho,
    \end{align*}
    which means that
    \begin{align*}
        % &=A\Big[(r+D-\rho)^{n-B} + \frac{1}{\rho(n-B+1)}[(r+D-\rho)^{n-B+1} - (r+D-k\cdot \rho)^{n-B+1}]\Big]\\
        \left(13\right)&\leq A\Big[\left(r+\D-\rho\right)^{d-B} + \frac{\left(\left(r+\D-\rho\right)^{d-B+1} - \rho^{d-B+1}\right)}{\rho\left(d-B+1\right)}\Big].
    \end{align*}
    Returning to our original expression and setting $\Tilde{r}:=r+D-\rho$, we get
    \begin{align*}
        &\sum_{i=1}^{[\frac{r+\D}{\rho}]-1} \left(\frac{I_\Lambda Vol\left(\B_1\right)}{2^d\sqrt{d}}\left(r+\D-i\rho\right)^d+a\frac{I_\Lambda}{2^d}\left(r+\D-i\rho\right)^{d-2}\right)\\
        &\leq \frac{I_\Lambda Vol\left(\B_1\right)}{2^d\sqrt{d}}\Big[\Tilde{r}^d\left(1+\frac{\Tilde{r}}{\rho \left(d+1\right)}\right) - \frac{\rho^d}{\left(d+1\right)}\Big] + \\
        &\qquad a\frac{I_\Lambda}{2^d}\Big[\Tilde{r}^{d-2}\left(1+\frac{\Tilde{r}}{\rho\left(d-1\right)}\right) - \frac{\rho^{d-2}}{d-1}\Big] \\
        &\leq \frac{I_\Lambda Vol\left(\B_1\right)}{2^d\sqrt{d}}\Big[\Tilde{r}^d\left(1+\frac{\Tilde{r}}{\rho \left(d+1\right)}\right)\Big] +
        a\frac{I_\Lambda}{2^d}\Big[\Tilde{r}^{d-2}\left(1+\frac{\Tilde{r}}{\rho \left(d-1\right)}\right)\Big].
    \end{align*}
    Because this refers to the unscaled space, we now want to move back to our rescaled space, using $\btheta$ and getting
    \begin{align*}
        &\frac{I_\Lambda Vol\left(\B_1\right)}{2^d\sqrt{d}}\Big[\btheta^d\left(1+\frac{\btheta}{\rho \left(d+1\right)}\right)\Big] +
        a\frac{I_\Lambda}{2^d}\Big[\btheta^{d-2}\left(1+\frac{\btheta}{\rho \left(d-1\right)}\right)\Big] \\
        &\leq \frac{I_\Lambda}{2^d}\btheta^{d-2}\left(1+\frac{\btheta}{\rho \left(d-1\right)}\right)\left(\frac{Vol\left(\B_1\right)}{\sqrt{d}}\btheta^2 + a\right).
    \end{align*}
    \itai{Here is another way, that reaches a DIFFERENT result for some reason}
    SECOND proof: 
    \begin{align*}
        &A\sum_1^k \left(r+\D-i\cdot \rho\right)^{d-B} \\
        = &A(r+\D-\rho)^{d-B}\sum_0^k \left(1-\frac{i\cdot \rho}{r+\D-\rho}\right)^{d-B} \\
    \end{align*}
    Let $x=\frac{i\cdot \rho}{r+\D-\rho}$. Then, $x>0$ (obvious, bc $\D >\rho\Rightarrow r+\D>\rho$). but also:
    \[
        x<1 \iff \frac{i\cdot \rho}{r+\D-\rho} < 1 \iff i<\frac{r+\D}{\rho}-1
    \]
    which is exactly what $k=[\frac{r+\D}{\rho}]-1$ holds, and $i\leq k$. From here, we use \({(1-x)^N<e^{-xN}}\) for $x\in(0,1)$:
    \begin{align*}
        \leq &A(r+\D-\rho)^{d-B}\sum_0^k e^{-\frac{i(d-B)\cdot \rho}{r+\D-\rho}} \\
        \leq &A(r+\D-\rho)^{d-B}\sum_0^{\infty} e^{-\frac{i(d-B)\cdot \rho}{r+\D-\rho}} \\
        = &A(r+\D-\rho)^{d-B} \left(1+\frac{1}{e^{\frac{(d-B)\cdot \rho}{r+\D-\rho}}}\right)\\
        \leq &2A(r+\D-\rho)^{d-B}
    \end{align*}
    At $r\rightarrow\infty$ we get $A(r+\D-\rho)^{d-B}$ instead of $2A\cdot(\dots)$.
    \itai{And just to contrast, the integral approximation got:}
    \begin{align*}
        \left(13\right)&\leq A\Big[\left(r+\D-\rho\right)^{d-B} + \frac{\left(\left(r+\D-\rho\right)^{d-B+1} - \rho^{d-B+1}\right)}{\rho\left(d-B+1\right)}\Big].
    \end{align*}
    \itai{this is much shorter than the other term, but also much better asymptotically. but I dont logically understand this. this means I can just ignore the sum alltogether. and then I get that the sum of length is pretty much the same order of magnitude as the number of samples, which makes no sense to me.}
    \itai{OK, I made a graph and appearently the number of samples IS proportional to the sum of edges! this is a test for a unit ball, I need to make sure its not a special case}

     \begin{figure}[H]
    \centering
    \includegraphics[width=0.66\linewidth]{Images/new_plot.png}
    \caption{proportional! }
    \label{fig:reflection}
\end{figure}

    Returning to the lattice basis $\{e_i\}$, we will now show that
    \[
        I_\Lambda=2^{d-2}\sum_i\|e_i\|^2.
    \]
    This is because
    \begin{align*}
        I_\Lambda &= \sum_{x\in P_{F_{\Lambda,p}}}\|x - c_{\Lambda,p}\|^2=_{[\ref{Lattice-properties}]} \sum_{x\in P_{F_{\Lambda,p}}}\|x - \frac{\sum e_i}{2}\|^2\\
        &=\sum_{a_i\in\{0,1\}}\|\sum_1^d a_i e_i -\frac{\sum e_i}{2}\|^2=\sum_{a_i\in\{0,1\}}\langle\sum_1^d\left(a_i-\frac{1}{2}\right)e_i,\sum_1^d\left(a_i-\frac{1}{2}\right)e_i\rangle\\
        &=\sum_{b_i\in \{\pm\frac{1}{2}\}} \sum_{i,j} b_ib_j\langle e_i,e_j\rangle= \sum_{b_i\in \{\pm\frac{1}{2}\}}b_i^2\sum_i\|e_i\|^2 + \sum_{b_i\in \{\pm\frac{1}{2}\}}\sum_{i\neq j}\langle e_i,e_j\rangle.
    \end{align*}
    We now notice two things: first, that $b_i^2=\frac{1}{4} \forall i$. Second, that for each $i,j$ there are 4 options: $\frac{1}{2},\frac{1}{2}$ and $-\frac{1}{2},-\frac{1}{2}$ which both lead to $\frac{1}{4}$, and $-\frac{1}{2},\frac{1}{2}$ and $\frac{1}{2},-\frac{1}{2}$ which both lead to $-\frac{1}{4}$. For that reason, all the terms of the second inner-product cancel each other out! We are left with:
    \begin{align*}
        \sum_{b_i\in \{\pm\frac{1}{2}\}}\frac{1}{4}\sum_i\|e_i\|^2=\frac{2^d}{4}\sum_i\|e_i\|^2=2^{d-2}\sum_i\|e_i\|^2,
    \end{align*}
    inserting this into the expression, we get our final version:
    \begin{align*}
        I\left(r\right)&\leq \frac{I_\Lambda}{2^d}\btheta^{d-2}\left(1+\frac{\btheta}{\rho \left(d-1\right)}\right)\left(\frac{Vol\left(\B_1\right)}{\sqrt{d}}\btheta^2 + a\right)\\
        &= \frac{1}{4}\left(\sum_i\|e_i\|^2\right) \btheta^{d-2}\left(\frac{\btheta}{\rho \left(d-1\right)}+1\right)\left(\frac{Vol\left(\B_1\right)}{\sqrt{d}}\btheta^2+ a\right).
    \end{align*}
\end{proof}
\end{proof}

    First, notice that the first two terms form a telescopic sum, which leaves us with
    \begin{align}
        =r^{N+1} - (r-\frac{[(r-r_0)n]}{rn})^{N+1} - \frac{1}{n}\sum_{i=0}^{[rn]-1}(r-\frac{i+1}{n})^N\nonumber\\        
        \leq r^{N+1} - r_0^{N+1} -\frac{1}{n}\sum_{i=0}^{[(r-r_0)n]-1}(r-\frac{i+1}{n})^N.
    \end{align}
    Looking at the second term, we can say that
    \begin{align*}
        \frac{1}{n}\sum_{i=0}^{[(r-r_0)n]-1}(r-\frac{i+1}{n})^N=\frac{r^N}{n}\sum_{i=0}^{[(r-r_0)n]-1}(1-\frac{i+1}{rn})^N=\frac{r^N}{n}\sum_{i=1}^{[(r-r_0)n]}(1-\frac{i}{rn})^N.
    \end{align*}
    Letting \(x=\frac{i}{rn}\), we trivially know that $x>0$, but we also know that
    \[
        x<1 \iff \frac{i}{rn} < 1 \iff i < rn,
    \]
    and surely enough \(i<[(r-r_0)n]<(r-r_0)n<rn\). This means we can use the bound of \({(1-x)^N>e^{\frac{-Nx}{1-x}}}\), getting
    \begin{align*}
        &\frac{r^N}{n}\sum_{i=1}^{[(r-r_0)n]}(1-\frac{i}{rn})^N\geq\frac{r^N}{n}\sum_{i=1}^{[(r-r_0)n]}e^{-N\frac{\frac{i}{rn}}{1-\frac{i}{rn}}}\\
        =&\frac{r^N}{n}\sum_{i=1}^{[(r-r_0)n]}e^{-N\frac{i}{rn-i}}.
    \end{align*}
    But we know that $i<(r-r_0)n\Rightarrow r_0n<rn-i$, which means that ${e^{-N\frac{i}{rn-i}}>e^{-N\frac{i}{r_0n}}}$. Using this with the formula for a geometric sum, we get
    \begin{align*}
        >&\frac{r^N}{n}\sum_{i=1}^{[(r-r_0)n]}e^{-N\frac{i}{r_0n}}= \frac{r^N}{n}\sum_{i=1}^{[(r-r_0)n]}\left(e^{\frac{-N}{r_0n}}\right)^i\\
        =&\frac{r^N}{n}\frac{e^{-\frac{[(r-r_0)n]N}{rn}} - e^{-\frac{N}{r_0n}}}{e^{-\frac{N}{r_0n}} - 1}\\
    \end{align*}
    and since $[(r-r_0)n]<(r-r_0)n$, we get
    \begin{align*}
        >& \frac{r^N}{n}\frac{e^{-\frac{(r-r_0)nN}{rn}} - e^{-\frac{N}{r_0n}}}{e^{-\frac{N}{r_0n}} - 1}
        = \frac{r^N}{n}\frac{e^{-\frac{(r-r_0)N}{r}} - e^{-\frac{N}{r_0n}}}{e^{-\frac{N}{r_0n}} - 1}\\
        =& r^N\frac{\frac{1}{n}}{e^{-\frac{N}{r_0n}} - 1}\left(e^{-\frac{(r-r_0)N}{r}} - e^{-\frac{N}{r_0n}}\right).
    \end{align*}
    First, we can quickly say that
    \[
        \lim_{n\rightarrow\infty}\left(e^{-\frac{(r-r_0)N}{r}} - e^{-\frac{N}{r_0n}}\right)=e^{-\frac{(r-r_0)N}{r}} - 1.
    \]
    Second, notice that
    \[
        \lim_{n\rightarrow\infty}\frac{\frac{1}{n}}{e^{-\frac{N}{r_0n}} - 1}=\frac{0^+}{0^-},
    \]
    meaning we can use the L'H\^ospital rule, getting
    \[
    \lim_{n\rightarrow\infty}\frac{\frac{1}{n}} {e^{\frac{-N}{r_0n}} - 1}
    =\lim_{n\rightarrow\infty}\frac{\frac{-1}{n^2}}{\frac{N}{r_0n^2}e^{\frac{-N}{r_0n}}}=\frac{-r_0}{N}\lim_{n\rightarrow\infty}e^{\frac{N}{r_0n}}=\frac{-r_0}{N}.
    \]
    Summarizing, using (10) with the above we get
    \begin{align}
        \sum_{i=0}^{[(r-r_0)n]-1} \left(r_i^{N+1} - r_ir_{i+1}^N\right)\leq& r^{N+1} - r_0^{N+1} -\frac{1}{n}\sum_{i=0}^{[(r-r_0)n]-1}(r-\frac{i+1}{n})^N\nonumber\\
        \leq&r^{N+1} - r_0^{N+1} - \left(r^N\cdot\frac{-r_0}{N}\left(e^{-\frac{(r-r_0)N}{r}} - 1\right)\right)\nonumber\\
        =& r^{N+1} - r_0^{N+1} - r^N\cdot\frac{r_0}{N}\left(1 - e^{-\frac{(r-r_0)N}{r}}\right).
    \end{align}
    Let $f(r_0):=r_0\left(1 - e^{-\frac{(r-r_0)N}{r}}\right)=r_0\left(1 - e^{\frac{N}{r}r_0-N}\right)$. We need to choose $r_0$ so that $f(r_0)$ gets a maximal value, causing the whole expression get the lowest value - resulting in the tightest bound. Let us solve it:
    \begin{align*}
        0&=\frac{d}{dr_0}f(r_0)=\left(1 - e^{\frac{N}{r}r_0-N}\right) - r_0\cdot e^{\frac{N}{r}r_0-N}\cdot \frac{N}{r}\\
        1&=e^{\frac{N}{r}r_0-N}(\frac{N}{r}r_0+1) \Rightarrow e^{N+1}=e^{\frac{N}{r}r_0+1}\left(\frac{N}{r}r_0+1\right).
    \end{align*}
    This type of equation, i.e.
    \[
        x=ye^y,x>0,
    \]
    has a solution $y=W_0(x)$ called a \emph{Lambert W function}. So, we get
    \begin{align*}
        \frac{N}{r}r_0+1=W_0(e^{N+1})\Rightarrow 
        r_0=\frac{r}{N}\left(W_0(e^{N+1})-1\right)
    \end{align*}
    as the value for the maximum. \itai{add check that it is indeed a maximum..} Let us use this equation again to get
    \begin{align*}
        \frac{N}{r}r_0+1=W_0(e^{N+1}) 
        \Rightarrow& \frac{N}{r}r_0-N=W_0(e^{N+1})-N-1\\
        \Rightarrow& e^{\frac{N}{r}r_0-N}=e^{W_0(e^{N+1})}e^{-(N+1)},
    \end{align*}
    but by definition
    \[
        W_0(e^{N+1})e^{W_0(e^{N+1})}=e^{N+1}\Rightarrow W_0(e^{N+1})=\frac{e^{N+1}}{W_0(e^{N+1})},
    \]
    which means that
    \begin{align*}
        e^{\frac{N}{r}r_0-N}=e^{W_0(e^{N+1})}e^{-(N+1)}=\frac{e^{N+1}}{W_0(e^{N+1})}e^{-(N+1)}=\frac{1}{W_0(e^{N+1})}.
    \end{align*}
    From here we can calculate the maximal $f$ value, getting
    \begin{align*}
        f(r_0) =& r_0\left(1 - e^{\frac{N}{r}r_0-N}\right) \\
        \leq& \frac{r}{N}\left(W_0(e^{N+1})-1\right)(1-\frac{1}{W_0(e^{-(N+1)})})\\
        =&\frac{r}{N}(W_0(e^{N+1})-1 - 1+\frac{1}{W_0(e^{-(N+1)})})\\
        =&\frac{r}{N}(W_0(e^{N+1})+\frac{1}{W_0(e^{-(N+1)})}-2)\\
        =&\frac{r}{N}(a_N+\frac{1}{a_N}-2), a_N:=W_0(e^{N+1}).
    \end{align*}
    Returning to (11), we get the expression
    \[
        (11) \leq r^{N+1} - r_0^{N+1} - \frac{r^N}{N}\left[\frac{r}{N}(a_N+\frac{1}{a_N}-2)\right].
    \]
    Remember that after summing the annulus we add the inner $r_0$-ball, which causes our final expression to be
    \[
        \leq r^{N+1} - \frac{r^{N+1}}{N^2}(a_N+\frac{1}{a_N}-2)=r^{N+1}\left(1-\frac{a_N+\frac{1}{a_N}-2}{N^2}\right)
    \]

In order that we do get better evaluations for each lattice, we will need to calculate $\D, \rho, \sum_i \|e_i\|^2$. Notice that, so far, this was done for a general lattice. Each lattice will differentiate by these values.
Using this theorem, we move on to our second contribution for this section.
\begin{thm}[\Lattices collision complexity]\label{collision_complexity_results}
    Fix $\beta=\beta\left(\delta,\epsilon\right)$ and $\theta:=\theta\left(\beta,R\right)$ as used previously. Consider the configuration space  $\C=\B_R$ and some $r$-ball $\B_r\subseteq\C$. Assume $\beta\leq1$ and $R\leq\sqrt{d}$. Then the following bounds hold:
    \begin{enumerate}[topsep=1pt,itemsep=1ex,partopsep=1ex,parsep=1ex]
        \item 
            $\text{CC}\left(\XZ\cap\B_r\right) \approx O\left(\frac{\beta}{\sqrt{d}}\left(\theta\left(\beta,r\right)\sqrt{\frac{d}{4}}+\sqrt{d}-\frac{1}{2}\right)^{d-1}\right)$
        \item 
            $\text{CC}\left(\XD\cap\B_R\right) \approx O\left(\frac{\beta}{\sqrt{d}}\left(\frac{r}{\beta}\sqrt{\frac{d}{8}-\frac{1}{16}}+\sqrt{\frac{9}{4}d}-\frac{1}{2}\right)^{d-1}\right)$
        \item 
            $\text{CC}\left(\XD\cap\B_R\right) \approx O\left(\frac{\beta}{\sqrt{d}}\left(\frac{r}{\beta}\sqrt{\frac{d}{12}}+\sqrt{d}-\frac{1}{2}\right)^{d-1}\right)$
    \end{enumerate}
\end{thm}
\begin{proof}
    First note that assuming our C-Space has $R\leq \sqrt{d}$ is reasonable, because
        \[
        \sqrt{d}\geq R\geq d\beta\Rightarrow\beta\leq\frac{1}{\sqrt{d}},
    \]
    and taking $d=10$ (similarly to our example in theorem~\ref{sample_lower}) requires us to have $\beta\leq 0.32$---similar to the situation in theorem~\ref{sample_lower}, which we explained makes sense.

    
    As mentioned before, we need to determine $\D, \rho, \sum_i \|e_i\|^2$ for each lattice. We get $I_\Lambda$ using all our previous knowledge. Regarding the inradius, Burchard et al.~\cite{burchard2015perimeter} gives us a lower bound for the inradius:
        \[
        \rho \geq Det\left(e_1,\dots,e_n\right) = \sqrt{\det\left(\Lambda\right)}
    \]
    The first term is the determinant of the lattice's base vectors. This is the volume of $F_\Lambda$, which is also a size given to us by Conway~\cite{conway2013sphere} as $\sqrt{\delta\left(\Lambda\right)}$. Finally, the diameter of each lattice will be determined using \cref{lemma:diameter}. Let us move on to our analysis of the lattices. Note that we will be using the shortened version of the approximation
    \[
        I\left(r\right)\approx O\left(\frac{\sum_i\|e_i\|^2}{\rho\left(d-1\right)}\btheta^{d-1}\right).
    \]
    because, as explained above, $Vol\left(\B_1\right)$ goes to 0 very quickly and becomes irrelevant.


    First, we look at $\ZN$. Using theorem \ref{thm:decomp_lattices} we know that our basis is 
    \[
        c\cdot e_i=c\cdot\left(0,\dots,1,\dots,0\right),
    \]
    for $c=\frac{2\beta}{\sqrt{d}}$. Being that the FRs are squares, the inradius is naturally exactly $\rho=\frac{c}{2}=\frac{\beta}{\sqrt{d}}$. 
    For the diameter, in a cube the longest distance is between the two "corners" (i.e. $(0,\dots,0)$ and $(1,\dots,1)$), so our diameter is
    \begin{align*}
        D&=c\|\left(1,\dots,1\right)\|\\
        &=c\sqrt{d}=\frac{2\beta}{\sqrt{d}}\sqrt{d}=2\beta.
    \end{align*}
    Lastly, we can see that 
    \[
        \sum_i \|e_i\|^2 =c^2d=\frac{4\beta^2}{d}d=4\beta^2,
    \]
    which gives us
    \begin{align*}
        &\frac{\sum_i\|e_i\|^2}{\rho\left(d-1\right)}=
        \frac{4\beta^2}{\frac{\beta}{\sqrt{d}}\left(d-1\right)}=\frac{4\beta\sqrt{d}}{d-1}.
    \end{align*}
    We now calculate $\btheta$ using the previous calculations and theorem~\ref{thm:decomp_lattices}, getting
    \begin{align*}
        \btheta &= \frac{r+D-\rho}{\beta}f_{\ZN}\\
        &= \frac{r+2\beta - \frac{\beta}{\sqrt{d}}}{\beta}\frac{\sqrt{d}}{2}\\
        & = \frac{r}{\beta}\frac{\sqrt{d}}{2}+\sqrt{d}-\frac{1}{2}.
    \end{align*}
    With these two calculations we get the final complexity
    \begin{align*}
        I\left(r\right)&\approx O\left(\frac{\sum_i\|e_i\|^2}{\rho\left(d-1\right)}\btheta^{d-1}\right)\\
        &=O\left(\frac{4\beta\sqrt{d}}{d-1}\left(\frac{r}{\beta}\frac{\sqrt{d}}{2}+\sqrt{d}-\frac{1}{2}\right)^{d-1}\right)\\
        &=O\left(\frac{\beta}{\sqrt{d}}\left(\frac{r}{\beta}\frac{\sqrt{d}}{2}+\sqrt{d}-\frac{1}{2}\right)^{d-1}\right)\\
        &=O\left(\frac{\beta}{\sqrt{d}}\left(\theta\left(\beta,r\right)\sqrt{\frac{d}{4}}+\sqrt{d}-\frac{1}{2}\right)^{d-1}\right).
    \end{align*}
    Next we look at $\DN$, using the base we got from theorem~\ref{thm:decomp_lattices}---the base vectors are $c\left(1,0,\dots,0\right)$ to $c\left(0,\dots,0,1,0\right)$ and $c\left(\frac{1}{2},\dots,\frac{1}{2}\right)$, with $c=\frac{4\beta}{\sqrt{2d-1}}$ (WLOG, $d$ is odd). We know from Conway~\cite{conway2013sphere} (page 120) that $\rho=\frac{1}{2}$, so after rescaling the space, we get $\frac{2\beta}{\sqrt{2d-1}}$. Next, our base vectors are all in the $[\mathbb{R}_+,\dots,\mathbb{R}_+]$ quadrant, so naturally (similar to the "cube" case!) the longest distance between any two points in the FR has to be between $\overset{\rightarrow}{0}$ and $\sum_i e_i$, getting that our diameter is
    \begin{align*}
        D&=c\|\left(1,0,\dots,0\right) + \dots + \left(0,\dots,1,0\right)+\left(\frac{1}{2},\dots,\frac{1}{2}\right)\|\\
        &=\frac{c}{2}\|\left(3,3,\dots,3,1\right)\|=\frac{c}{2}\sqrt{9\left(d-1\right)+1}\\
        &=\frac{c}{2}\sqrt{9d-8}=2\beta\sqrt{\frac{9d-8}{2d-1}}.
    \end{align*}
    Lastly, we can see that 
    \begin{align*}
        &\sum_i \|e_i\|^2 =c^2\left(d-1\right)+c^2\frac{d}{4}=\frac{c^2}{4}\left(5d-4\right)\\
        &=\frac{4\beta^2}{2d-1}\left(5d-4\right)=
        4\beta^2\frac{\left(5d-4\right)}{2d-1},
    \end{align*}
    which gives us
    \begin{align*}
        &\frac{\sum_i\|e_i\|^2}{\rho\left(d-1\right)}=
        \frac{4\beta^2\frac{\left(5d-4\right)}{2d-1}}{\frac{2\beta}{\sqrt{2d-1}}\left(d-1\right)}\\
        &=2\beta\frac{\sqrt{2d-1}\left(5d-4\right)}{\left(d-1\right)\left(2d-1\right)}.
    \end{align*}
    We now calculate $\btheta$ using the previous calculations and theorem~\ref{thm:decomp_lattices}, getting
    \begin{align*}
        \btheta &= \frac{r+D-\rho}{\beta}f_{\DN}\\
        &= \frac{r+2\beta\sqrt{\frac{9d-8}{2d-1}}-\frac{2\beta}{\sqrt{2d-1}}}{\beta}\frac{\sqrt{2d-1}}{4}\\
        &= \frac{r}{\beta}\frac{\sqrt{2d-1}}{4}+\sqrt{\frac{9}{4}d-2}-\frac{1}{2}.
    \end{align*}
    With these two calculations we get the final complexity
    \begin{align*}
        I\left(r\right)&\approx O\left(\frac{\sum_i\|e_i\|^2}{\rho\left(d-1\right)}\btheta^{d-1}\right)\\
        &=O\left(2\beta\frac{\sqrt{2d-1}\left(5d-4\right)}{\left(d-1\right)\left(2d-1\right)}\left(\frac{r}{\beta}\frac{\sqrt{2d-1}}{4}+\sqrt{\frac{9}{4}d-2}-\frac{1}{2}\right)^{d-1}\right)\\
        &=O\left(\frac{\beta\sqrt{d-\frac{1}{2}}}{d-1}\left(\frac{r}{\beta}\sqrt{\frac{d}{8}-\frac{1}{16}}+\sqrt{\frac{9}{4}d-2}-\frac{1}{2}\right)^{d-1}\right)\\
        &=O\left(\frac{\beta}{\sqrt{d}}\left(\frac{r}{\beta}\sqrt{\frac{d}{8}-\frac{1}{16}}+\sqrt{\frac{9}{4}d}-\frac{1}{2}\right)^{d-1}\right)\\
    \end{align*}
    Finally, we look at $\AN$. The base we got from theorem~\ref{thm:decomp_lattices} uses the vectors $\left(c,-c,0\dots,0\right)$ to $\left(c,0,\dots,0,-c,0\right)$ and $\left(\frac{-cd}{d+1},\frac{c}{d+1}\dots,\frac{c}{d+1}\right)$ for $c=\sqrt{\frac{12\left(d+1\right)}{d\left(d+2\right)}}\beta$. As our method relies on the diameter of the FR, and this FR's diameter is roughly $O\left(d\right)$ (due to the first coordinate being filled on all vectors) in contrast to $O\left(\sqrt{d}\right)$ in the other lattices, we will use a different FR: we will use
    \begin{align*}
        v_1&=\left(c,-c,0,\dots,0\right)\\
        v_2&=\left(0,c,-c,\dots,0\right)\\
        v_d&=\left(0,\dots,0,c,-c,0\right)\\
        w&=\left(\frac{-cd}{d+1},\frac{c}{d+1}\dots,\frac{c}{d+1}\right).
    \end{align*}
    This spans the same lattice, as we can recreate the original basis from this (by adding $i$ vectors in a row).  To calculate the inradius, we refer to pages LXII and 10 of Conway~\cite{conway2013sphere}, citing that 
    \[
        \rho = \left(\delta\sqrt{\det{\Lambda}}\right)^{\frac{1}{d}},
    \]
    where $\delta$ is a parameter given in page 115 which is independent of choice of basis. The only thing left to calculate, then, is $\det{\Lambda}=det\left(G_\Lambda G_\Lambda^t\right)$. Let us calculate it:
    \begin{align*}
        \det{\Lambda}&=det\left(G_\Lambda G_\Lambda^t\right)\\
        &=\det\begin{pmatrix}
            1 & -1 &  0  & \dots & 0 & 0 & 0 \\
            0 & 1  &  -1 & \dots & 0 & 0 & 0 \\
            . & .  &  . & \dots & . & .  & .\\
            0 & 0  &  0 & \dots & 1 & -1 & 0\\
            \frac{-d}{d+1} & \frac{1}{d+1} & \frac{1}{d+1} & \dots & \frac{1}{d+1} & \frac{1}{d+1} & \frac{1}{d+1}
        \end{pmatrix}
        \begin{pmatrix}
            1 & 0 & \dots & 0 & 0 & \frac{-d}{d+1} \\
            -1 & 1 & \dots & 0 & 0 & \frac{1}{d+1} \\
            0 & -1 & \dots & 0 & 0 & \frac{1}{d+1} \\
            . & . & \dots & . & .  & .\\
            0 & 0 & \dots & 0 & -1 & \frac{1}{d+1}\\
            0 & 0 & \dots & 0 & 0 & \frac{1}{d+1}
        \end{pmatrix}\\
        &=\det\begin{pmatrix}
            2 & -1 &  0  & 0 & 0 &\dots & 0 & 0 & -1\\
            -1 & 2  &  -1 & 0 & 0 &\dots & 0 & 0 & 0\\
            0 & -1  &  2 & -1 & 0 & \dots & 0 & 0 & 0\\
            . & .  &  . & . & . & \dots & . & . & .\\
            0 & 0  &  0 & 0 & 0 & \dots & -1 & 2 & 0\\
            -1 & 0  &  0 & 0 & 0 &\dots & 0 & 0 & \frac{d}{d+1}\\
        \end{pmatrix},\\
    \end{align*}
    now add all $d-1$ rows to the last row:
    \begin{align*}
        &=\det\begin{pmatrix}
            2 & -1 &  0  & 0 & 0 &\dots & 0 & 0 & -1\\
            -1 & 2  &  -1 & 0 & 0 &\dots & 0 & 0 & 0\\
            0 & -1  &  2 & -1 & 0 & \dots & 0 & 0 & 0\\
            . & .  &  . & . & . & \dots & . & . & .\\
            0 & 0  &  0 & 0 & 0 & \dots & -1 & 2 & 0\\
            0 & 0  &  0 & 0 & 0 &\dots & 0 & 1 & \frac{d}{d+1}-1\\
        \end{pmatrix}.
    \end{align*}
    We now cancel out the first non-zero coordinate in the second row using the first row, and then multiply it by an integer so it becomes an integer row, getting
    \begin{align*}
        &=\det\begin{pmatrix}
            2 & -1 &  0  & 0 & 0 &\dots & 0 & 0 & -1\\
            0 & 1.5  &  -1 & 0 & 0 &\dots & 0 & 0 & 0.5\\
            0 & -1  &  2 & -1 & 0 & \dots & 0 & 0 & 0\\
            . & .  &  . & . & . & \dots & . & . & .\\
            0 & 0  &  0 & 0 & 0 & \dots & -1 & 2 & 0\\
            0 & 0  &  0 & 0 & 0 &\dots & 0 & 1 & \frac{d}{d+1}-1\\
        \end{pmatrix}\\
        &=\frac{1}{2}\det\begin{pmatrix}
            2 & -1 &  0  & 0 & 0 &\dots & 0 & 0 & -1\\
            0 & 3  &  -2 & 0 & 0 &\dots & 0 & 0 & -1\\
            0 & -1  &  2 & -1 & 0 & \dots & 0 & 0 & 0\\
            . & .  &  . & . & . & \dots & . & . & .\\
            0 & 0  &  0 & 0 & 0 & \dots & -1 & 2 & 0\\
            0 & 0  &  0 & 0 & 0 &\dots & 0 & 1 & \frac{d}{d+1}-1\\
        \end{pmatrix}.
    \end{align*}
    we keep going like this recursively
    \begin{align*}
            &=\frac{1}{2}\det\begin{pmatrix}
            2 & -1 &  0  & 0 & 0 &\dots & 0 & 0 & -1\\
            0 & 3  &  -2 & 0 & 0 &\dots & 0 & 0 & -1\\
            0 & 0  &  \frac{4}{3} & -1 & 0 & \dots & 0 & 0 & \frac{-1}{3}\\
            . & .  &  . & . & . & \dots & . & . & .\\
            0 & 0  &  0 & 0 & 0 & \dots & -1 & 2 & 0\\
            0 & 0  &  0 & 0 & 0 &\dots & 0 & 1 & \frac{d}{d+1}-1\\
        \end{pmatrix},
    \end{align*}
    until ultimately, we reach the last row, getting
    \begin{align*}
        &=\frac{1}{\left(d-1\right)!}\det\begin{pmatrix}
            2 & -1 &  0  & 0 & 0 &\dots & 0 & 0 & -1\\
            0 & 3  &  -2 & 0 & 0 &\dots & 0 & 0 & -1\\
            0 & 0  &  4 & -3 & 0 & \dots & 0 & 0 & -1\\
            . & .  &  . & . & . & \dots & . & . & .\\
            0 & 0  &  0 & 0 & 0 & \dots & 0 & d & -1\\
            0 & 0  &  0 & 0 & 0 &\dots & 0 & 1 & \frac{d}{d+1}-1\\
        \end{pmatrix}\\
        &=\frac{1}{\left(d-1\right)!}\det\begin{pmatrix}
            2 & -1 &  0  & 0 & 0 &\dots & 0 & 0 & -1\\
            0 & 3  &  -2 & 0 & 0 &\dots & 0 & 0 & -1\\
            0 & 0  &  4 & -3 & 0 & \dots & 0 & 0 & -1\\
            . & .  &  . & . & . & \dots & . & . & .\\
            0 & 0  &  0 & 0 & 0 & \dots & 0 & d & -1\\
            0 & 0  &  0 & 0 & 0 &\dots & 0 & 0 & \frac{d}{d+1}-1+\frac{1}{d}\\
        \end{pmatrix}\\
        &=\frac{1}{\left(d-1\right)!}\cdot d!\left(\frac{1}{d\left(d+1\right)}\right)
        =\frac{1}{d+1}.
    \end{align*}    
    Looking at page 115 of~\cite{conway2013sphere}, we see that the determinant of the classic basis is similar to our FR's, which means we can just use the inradius for the classic basis, which is quoted to be
    \[
        \rho = \frac{1}{2}\sqrt{\frac{d}{d+1}},
    \]
    and after rescaling the space we get
    \[
        \rho=\frac{1}{2}\sqrt{\frac{d}{d+1}}\sqrt{\frac{12\left(d+1\right)}{d\left(d+2\right)}}\beta
        =\frac{1}{2}\sqrt{\frac{12}{d+2}}\beta.
    \]
    Next, to calculate the diameter we need to consider distances between all binary sums ("in the sum or not") of base vectors. If we add $v_i,v_{i+1}$ then the $i+1$-coordinate cancels out and we get $\left(\dots,1,0,-1,\dots\right)$. This lowers the possible contribution of this coordinate, as it only appears in these vectors and in $w$, and in $w$ it is $\frac{-1}{d+1}$---resulting in a total of $\frac{1}{d+1}$ (in absolute value). This is in contrast to adding $v_i,v_j$ where $j\geq i+2$, so we get $\left(\dots,1,-1,\dots,1,-1,\dots\right)$. When adding it to $w$ now, we get $1-\frac{1}{d+1}>\frac{1}{d+1}$ (in absolute value). So we see that in general, the longest difference between FR points we can get is when adding $u=w+v_1+v_3+v_5+\dots$, getting
    \begin{align*}
        D^2&=\|u\|^2=c^2\|\left(1,-1,1,-1,\dots,-1,0\right)+\left(\frac{-d}{d+1},\frac{1}{d+1},\dots,\frac{1}{d+1}\right)\|^2\\
        &=c^2\|\left(1-\frac{d}{d+1},-\left(1-\frac{1}{d+1}\right),1-\frac{1}{d+1},\dots,-\left(1-\frac{1}{d-1}\right),\frac{1}{d+1}\right)\|^2\\
        &=c^2\|\left(\frac{1}{d+1},-\left(1-\frac{1}{d+1}\right),1-\frac{1}{d+1},\dots,-\left(1-\frac{1}{d+1}\right),\frac{1}{d+1}\right)\|^2\\
        &=c^2\left(\frac{2}{\left(d+1\right)^2}+\frac{d}{2}\left(1-\frac{1}{d+1}\right)^2\right)\\
        &=\frac{1}{2}c^2\frac{4+d^3}{\left(d+1\right)^2},\\
        \Rightarrow D&=\frac{c}{\sqrt{2}}\frac{d}{d+1}\sqrt{d+\frac{4}{d^2}}\leq\frac{c}{\sqrt{2}}\sqrt{d+2}\\
        &=\frac{1}{\sqrt{2}}\sqrt{\frac{12\left(d+1\right)}{d\left(d+2\right)}}\beta\sqrt{d+1}=\sqrt{\frac{6\left(d+1\right)}{d}}\beta\leq\sqrt{12}\beta.
    \end{align*}
    Lastly, we can see that 
    \begin{align*}
        &\sum_i \|e_i\|^2 =c^2\left(d\cdot\left(2\right)+1\cdot\left(\frac{d^2}{\left(d+1\right)^2}+d\frac{1}{\left(d+1\right)^2}\right)\right)\\
        &=c^2\left(2d+\frac{d}{d+1}\right)
        = \frac{12\left(d+1\right)}{d\left(d+2\right)}\beta^2\left(2d+\frac{d}{d+1}\right)\\
        &\leq\frac{12}{d}\beta^2\left(2d+1\right)\leq 36\beta^2,
    \end{align*}
    which gives us
    \begin{align*}
        &\frac{\sum_i\|e_i\|^2}{\rho\left(d-1\right)}\leq
        \frac{36\beta^2}{\frac{1}{2}\sqrt{\frac{12}{d+2}}\beta\left(d-1\right)}\\
        &=\frac{36\beta\sqrt{d+2}}{\sqrt{3}\left(d-1\right)}.
    \end{align*}
    We now calculate $\btheta$ using the previous calculations and theorem~\ref{thm:decomp_lattices}, getting
    \begin{align*}
        \btheta &= \frac{r+D-\rho}{\beta}f_{\DN}\\
        &\leq \frac{r+\sqrt{12}\beta-\frac{1}{2}\sqrt{\frac{12}{d+2}}\beta}{\beta}\sqrt{\frac{d\left(d+2\right)}{12\left(d+1\right)}}\\
        &= \frac{r}{\beta}\sqrt{\frac{d\left(d+2\right)}{12\left(d+1\right)}}+\sqrt{\frac{d\left(d+2\right)}{\left(d+1\right)}}-\frac{1}{2}\sqrt{\frac{d}{\left(d+1\right)}}\\
        &=\sqrt{\frac{d+2}{d+1}}\left(\frac{r}{\beta}\sqrt{\frac{d}{12}}+\sqrt{d}-\frac{1}{2}\sqrt{\frac{d}{d+2}}\right).
    \end{align*}
    Remember that we have seen in corollary~\ref{cor:specific_sample_complexity} that $\left(\sqrt{\frac{d+2}{d+1}}\right)^d\rightarrow\sqrt{e}$. With  the calculations above, we get the final complexity
    \begin{align*}
        I\left(r\right)&\approx O\left(\frac{\sum_i\|e_i\|^2}{\rho\left(d-1\right)}\btheta^{d-1}\right)\\
        &=O\left(\frac{36\beta\sqrt{d+2}}{\sqrt{3}\left(d-1\right)}\left(\sqrt{\frac{d+2}{d+1}}\left(\frac{r}{\beta}\sqrt{\frac{d}{12}}+\sqrt{d}-\frac{1}{2}\sqrt{\frac{d}{d+2}}\right)\right)^{d-1}\right)\\
        &=O\left(\frac{\beta}{\sqrt{d}}\left(\sqrt{\frac{d+2}{d+1}}\right)^{d-1}\left(\frac{r}{\beta}\sqrt{\frac{d}{12}}+\sqrt{d}-\frac{1}{2}\sqrt{\frac{d}{d+2}}\right)^{d-1}\right)\\
        &=O\left(\frac{\beta}{\sqrt{d}}\left(\frac{r}{\beta}\sqrt{\frac{d}{12}}+\sqrt{d}-\frac{1}{2}\sqrt{\frac{d}{d+2}}\right)^{d-1}\right)\\
        &=O\left(\frac{\beta}{\sqrt{d}}\left(\frac{r}{\beta}\sqrt{\frac{d}{12}}+\sqrt{d}-\frac{1}{2}\right)^{d-1}\right)\\
    \end{align*}
\end{proof}
\subsection*{Comparing collision 
complexity for \Lattices}
The collision complexity of the lattices seems to be naturally "carried over" from the sample complexity. In this aspect, all conclusions we drew previously apply here: $\AN$ still rises as having the least total edge length, resulting in a lower amount of collision checks. The higher degree of the power in comparison to sample complexity ($d-1$ against $d-2$) means these differences are even more accentuated. 

\subsection*{Comparing $\AN$ to random sample sets}
 
 First thing we compared was the classic $PRM$ algorithm to our setting, with the purpose of seeing how $\AN$ stands against random sample sets, which are known to generally give good enough results. This test was conducted with a regular PRM algorithm, with the "H" map, at $d=6$ using 3 moving disks, with some augments that we will soon list. Just to note, we used a much higher clearance of $\delta=25$, which was found to empirically work with $\AN$. This high clearance value allows us also to see another facet of the LPRM issue: clearance rates are pivotal to having feasible runtimes in MPs. The following method was used in this test section:
 \begin{enumerate}
     \item Each of the three robots has a set location in a corner of the "H" map. 
     \item We create a test set this way: shift every robot a bit, into a legal position, by $N$ steps. This creates $N^3$ sets. Permute the three robots (we plan in a $d=3\cdot2=6$, so these are different tests), getting 6 test. Overall: $6N^3$ tests. We chose $N=3$ for 162 tests.
     \item On each of these tests, run two problems: first, a run of $\AN$ with LPRM. On finishing, save the length and solution time and get the number of samples used. Second, a run of PRM using a fixed amount of samples---the number we got from the LPRM run.
     \item The second test is then run in two different modes. First, we use LPRM's radius, the one used from Dayan et al.~\cite{dayan2023near}. Then we use PRM*'s radius. 
     \item What we look for are relative qualities (our data divided by their data) and success rates, all averaged over the 162 tests.
 \end{enumerate}
 Results: (all done at $\delta=25$)
 \begin{enumerate}
     \item \underline{Both with same radius:} 
     \begin{enumerate}
        \item Success rate: $\AN$ with LPRM: 100\%, random with PRM: $\epsilon=10$ with success=42\%, $\epsilon=5$ with success=53\%, $\epsilon=2$ with success=100\%.
        \item Total time quality, $\frac{\text{LPRM time}}{\text{rnd PRM time}}$: $\epsilon=10$ with quality=7.77, $\epsilon=5$ with quality=10.87, $\epsilon=2$ with quality=11.93.
        \item $A^*$ \textbf{run only} time quality, $\frac{A^*-\text{LPRM time}}{A^*-\text{rnd PRM time}}$: $\epsilon=10$ with quality=1.96, $\epsilon=5$ with quality=2.39, $\epsilon=2$ with quality=4.55.
        \item Length quality, $\frac{\text{LPRM length}}{\text{rnd PRM time}}$: $\epsilon=10$ with quality=1.25, $\epsilon=5$ with quality=1.22, $\epsilon=2$ with quality=1.13.
     \end{enumerate}
     \item \underline{Each with its own radius:}
          \begin{enumerate}
         \item Success rate: all 100\% at all values.
         \item Total time quality, $\frac{\text{LPRM time}}{\text{rnd PRM time}}$: $\epsilon=10$ with quality=1.12, $\epsilon=5$ with quality=1.3, $\epsilon=2$ with quality=3.96.
        \item $A^*$ \textbf{run only} time quality, $\frac{A^*-\text{LPRM time}}{A^*-\text{rnd PRM time}}$: $\epsilon=10$ with quality=1.2, $\epsilon=5$ with quality=1.64, $\epsilon=2$ with quality=4.13.
         \item Length quality, $\frac{\text{LPRM length}}{\text{rnd PRM time}}$: $\epsilon=10$ with quality=1.25, $\epsilon=5$ with quality=1.22, $\epsilon=2$ with quality=1.13.
     \end{enumerate}
 \end{enumerate}
%  \begin{figure*}[!h]
%   \centering
%   \subfloat[this image is a placeholder]{
%     \includegraphics[width=0.3\textwidth]{Images/CC_relative_by_e.png}
%     \label{fig:exp_3body:hmap}}
%   \hfil
%   \subfloat[this image is a placeholder]{
%     \includegraphics[width=0.3\textwidth]{Images/CC_relative_by_e.png}
%     \label{fig:exp_3body:rndpoly}}
%   \caption{The scenarios we used to test our sample set, in each map we wanted each disk-robot to switch places with the next neighbor.}
%   \label{fig:exp_3body}
% \end{figure*}

\emph{Second section conclusions:} there are several conclusions we can draw. 
\begin{enumerate}
    \item First, that if PRM isn't given a good enough sampling radius, then it will not find a solution a meaningful percentage of the time. This is in contrast to LPRM, which is deterministically guaranteed to get a result, after you pass certain sample density "threshold".
    \item Second, we can see that while rnd-PRM had a better average path quality, it was not substantial (at worse 2x longer).
    \item Lastly, it is clear that rnd-PRM is quicker than LPRM, which is to be expected: we have much more edges in LPRM than in rnd-PRM. This is true also in case we only count the $A^*$ runtime only (without the time to build the graph). In $\epsilon=10$ the runtimes do get very close, but in realistically lower $\epsilon$ values rnd-PRM is much quicker again.
\end{enumerate}

Overall, it is notable that LPRM has not demonstrated a significant improvement over rnd-PRM, at least in our setting. Its strengths lay in its theoretical promise to achieve a good result in finite time, in contrast to rnd-PRM. We will demonstrate in the next section the promise of the $\AN$ lattice over the others.

\subsection*{Comparing runtimes between the lattices}
 
 The second set of tests compared the lattices themselves: \Lattices. This version of LPRM saw two important improvements to the runtime, that greatly improved it.
 \begin{enumerate}
     \item The first one was to move to a fully "lazy" implementation, on a graph that already implicitly exists: we know in advance that each point in the lattice has $2d$ neighbors, and we know their location. Therefor we don't have to build the graph at all, and just consider the implicit neighbors. That is in contrast to a graph with random sampling, in which the graph is incrementally built as you add samples, which makes comparing to an implicit graph impossible.
     \item The second was to recognize that we can calculate a points neighbor's in a general ball, in advance, and then just have a point's neighbors be these same points - only shifted! This is due to the regularity of the lattice structure.
 \end{enumerate}
The results, each averaged over 6 different case, are as follows:

\begin{table*}[t]
\centering
\caption{LPRM vs RPRM, Both with the same radius (from Dayan~\cite{dayan2023near})}
\begin{tabularx}{\linewidth}{|X|X|X|X||X|X|X|X|X|X|X|X|X|} \hline
 Map & ID & Scenario & NN &
 \multicolumn{4}{|c|}{Construction times [S]} &
 \multicolumn{4}{|c|}{$A^*$ times [S]} &
  Success
 \\
 \hline
 & & & & $\ZN$ & $\DN$ & $\AN$ & Random & $\ZN$ & $\DN$ & $\AN$ & Random & \\
 \hline
 \multirow{4}{*}{K}
  & 1 & 2-Swap & No  & $0.0001$    &$9E(-5)$&   $9E(-5)$ & $2.308$ & $5.505$ & $2.212$ & \cellcolor{green} $1.214$ & \cellcolor{pink} $1.569$ & 100\%\\
  \cline{2-13}
  & 1 & 2-Swap & Yes  & $7.643$    &$3.897$&   $3.087$ & $2.308$ & $6.140$ & $2.468$ & \cellcolor{green}$1.363$ & \cellcolor{pink}$1.569$ & 100\%\\
  \cline{2-13}
  & 2& 3-Swap   & No & $0.0042$    &$0.0014$&   $0.0032$ & NA & $78.493$ & $10.391$ &\cellcolor{green} $3.786$ & \cellcolor{pink}NA & 0\% \\
    \cline{2-13}
  & 2& 3-Swap   & Yes & $0.0042$    &$0.0014$&   $0.0032$ & NA & $78.493$ & $10.391$ &\cellcolor{green} $3.786$ & \cellcolor{pink}NA & 0\% \\
 \hline
  \multirow{4}{*}{UM}
  & 3 & 2-Swap  & No & $0.00028$    &$0.00013$&   $0.00014$ & $1.061$ & $54.638$ & $17.463$ & \cellcolor{green}$7.316$ & \cellcolor{pink}$8.650$ & 100\% \\
  \cline{2-13}
    & 3 & 2-Swap  & Yes & $3.277$    &$1.799$&   $1.278$ & $1.061$ & $64.355$ & $19.701$ &\cellcolor{green} $8.346$ & \cellcolor{pink}$8.650$ & 100\% \\
  \cline{2-13}
  & 4& 3-Swap  & No & $0.00637$    &$0.001851$&   $0.000691$ & $40.972$ & $506.254$ & $25.898$ &\cellcolor{green} $7.029$ & \cellcolor{pink}$21.380$ & 95\% \\
    \cline{2-13}
    & 4& 3-Swap  & Yes & $437.237$    &$124.184$&   $68.451$ & $40.972$ & $912.857$ & $56.335$ & \cellcolor{pink}$21.774$ & \cellcolor{green}$21.380$ & 95\% \\
 \hline
 \multirow{4}{*}{RP}
  & 5& 2-Swap  & No & $0.000179$    &$0.000172$&   $0.450$ & $0.465$ & $5.532$ & $1.954$ & \cellcolor{green}$1.612$ & \cellcolor{pink}$2.323$ & 100\%\\
  \cline{2-13}
    & 5& 2-Swap  & Yes & $1.472$    &$0.770$&   $0.554$ & $0.465$ & $6.335$ & $2.185$ & \cellcolor{green}$1.672$ & \cellcolor{pink}$2.323$ & 100\%\\
  \cline{2-13}
  & 6 & 3-Swap  & No & $0.0062$    &$0.0020$&   $0.0007$ & $21.227$ & $812.614$ & $7.207$ & \cellcolor{pink}$7.347$ & \cellcolor{green}$5.833$ & 100\%\\
    \cline{2-13}
  & 6 & 3-Swap  & Yes & $225.829$    &$61.552$&   $33.688$ & $21.227$ & $1127.65$ & $9.771$ & \cellcolor{pink}$10.898$ & \cellcolor{green}$5.833$ & 100\%\\
 \hline
\end{tabularx}
\end{table*}

\begin{enumerate}
    \item \textbf{Test \#1}: d=6, $\delta=9, \epsilon=10$, "H" map, 3 disk robots $(x,y)$. Results:
    \begin{enumerate}
        \item Zn average total runtime: 1141 seconds.
        \item Dn* average total runtime: 55 seconds.
        \item An* average total runtime: 23 seconds.
    \end{enumerate}
    \underline{Conclusion:} $\AN$ runs 50x faster than $\ZN$.
    \item \textbf{Test \#2}: d=6, $\delta=??, \epsilon=10$, "random polygons" map, 3 disk robots $(x,y)$. Results:
    \begin{enumerate}
        \item Zn average total runtime: ?? seconds.
        \item Dn* average total runtime: ?? seconds.
        \item An* average total runtime: ?? seconds.
    \end{enumerate}
    \underline{Conclusion:} $\AN$ runs ?? faster than $\ZN$.
\end{enumerate}
\emph{First section conclusions:} it is clear from these comparisons that $\AN$ performs much better than $\ZN$. Another point to notice is the differences between the lattices: if we wanted an even lower clearance or stretch factor, $\ZN$'s runtime would become infeasible to run. We believe that if you are considering using a deterministic sample set, for any purpose, the set $\AN$ has demonstrated a substantial superiority over other lattices---making it a good choice to use.

==> tex/9_CC_bounds_old.tex <==
\section{Collision-check complexity}\label{sec:collision_complexity}
In this section, we seek to analyze the collision-check complexity of our sample sets $\XZ,\XD,\XA$, as the length of the graph edges is a better proxy for the computational complexity of constructing the resulting PRM than sample complexity. 

%The biggest effect on the runtime of a PRM algorithm are the collision checks. Specifically, running neighborhood checks (like r-NN) forces you to check along all the edges connecting the center of a ball with other vertices for the purpose of finding a possible collision.


%For this reason, we would like to have some estimate on the overall size of the sum of lengths from the ball center to the other vertices.
%
% To make calculations simpler, we'll use $\sum\|\cdot\|^2$ instead. \kiril{Note to self: Need to revise the definition of CC-complexity to account for this squared value and provide a motivation about it.}


%\itai{Some thoughts: this sum can also be seen as the Moment of inertia of a collection of particles of similar mass, scattered on a lattice inside a sphere. Is this useful to note? if anything, the connection could be interesting. In the beginning I tried to find some way to connect the two, as I thought maybe physicists already have estimates for this kind of thing. For example, the Dn* lattice in d=2 is known to be a crystal lattice for some materials. is our calculation getting the approximate moment of inertia for a pure crystal ball? checking online, iron for example is a BCC crystal. so a crystal iron ball has a moment of $0.4Mr^2$, and you'll see later we reach O($r^2$) approximately. I just wonder if we should point out the connection at any point, even as a comparison.} \kiril{This is interesting. We could point out this connection, in a more concise manner, after Problem 2. This could definitely go into the thesis.}


% Next, introduce a few more definitions that are closely related to the  collision-check complexity bounds.
Recall that the collision-check complexity of a lattice-based sample set $\X_\Lambda$  is 
$CC_{\X_\Lambda}=\sum_{x\in \X_\Lambda\cap \B_r}\|x\|$, where $r=r(\delta,\eps)$.
A naive approach to upper-bound $CC_{\X_\Lambda}$ is to multiply the number of points in a $r$-ball (which corresponds to the sample complexity of $\X_\Lambda$) with the radius $r$, i.e.,
\begin{align}
    CC_{\X_\Lambda}\leq r\cdot |X_\Lambda \cap \B_r|=r\cdot \frac{\partial(B_1)}{\sqrt{\det(\Lambda)}}\btheta^d_r + r\cdot P_d(\btheta_r). \label{eq:cc_naive}
\end{align}
The following is a tighter bound, which reduces the coefficient of the dominant factor of the naive bound.  

%A tighter bound can be obtained by partitioning the $r$-ball into annuli and separately counting the distances to the points in a given annulus. %In the proof below, for simplicity, we use the bound  $P_d(\btheta)=\Theta(\btheta^{d-2})$, which is applicable to any dimension $d\geq 3$, even though tighter bounds are available for $d\in \{3,4\}$.

%That is, an annulus is defined as  $A^{r'}_{r''}:=\B_{r'}(o)\setminus \B_
%{r''}(o)$ for some $0\le r''<r'\le r$, and  the distances corresponding to this annulus are $r' \cdot |\X\cap A^{r'}_{r''}|$. Note that the expression $|\X\cap A^{r'}_{r''}|$ can be approximated via Equation~\ref{eq:sample bounds} by subtracting from the upper bound of $|\X\cap \B_{r'}(o)|$ the lower bound of $|\X\cap \B_{r''}(o)|$. However, this should be done carefully since this method can yield a strictly positive number of points for an annulus of zero width due to the slackness in Equation~\ref{eq:sample bounds}. We have the following theorem.

%\begin{definition}[Ball collision complexity]\label{def:lattice_sums}
%  Let \(P_{\Lambda,r}:= \{\Lambda\cap \B_r\left(0\right)\}\) be the lattice $\Lambda$ points inside the $r$-ball centered at $o$, for some $r\geq 0$. The \emph{collision complexity} of $P_r$ is defined to be
%   $$\text{CC}_{\Lambda}\left(r\right):=\sum_{x\in P_{\Lambda,r}} \|x\|.$$
% Also, let \(P_{F_{\Lambda,p}}:=F_{\Lambda,p}\cap \Lambda\) be the lattice samples that belong to an FR $F_{\Lambda,p}$, and consider another FR $F_{\Lambda,p'}$ where both FRs are defined with the same basis of $\Lambda$, where $p,p'\in \dR^d$. \kiril{I made some clarifications. Are they correct?}
% We define the relative sum to be the squared distance of the points in $P_{F_{\Lambda,p}}$ from the center $c_{\Lambda,p'}$ of $F_{\Lambda,p'}$, i.e.,
%         \[
%            I_{F,p'}:=\sum_{x\in P_{F}} \|c_{\Lambda,p'}-x\|^2.
%           %I_{F_{\Lambda,p}}=
%         \]
%\end{definition}

% Using these definitions, we work towards bounding \(I\left(r\right)\), which would then lead to collision-check complexity bounds. 

\begin{thm}[CC complexity bound]
  Consider a lattice $\Lambda\in \{\dZ^d,D_d^*,A_d^*\}$ with a covering radius $f_\Lambda$, which yields the \decomp set $\X:=\XL$ for some $\delta>0,\epsilon>0$ and dimension $d\geq 3$ \kiril{Shouldn't it be dimension 2 and on?}. %Fix a radius $R>0$.\footnote{Notice that since the connection radius we use is $r:=r(\delta,\epsilon)$, we could potentially limit $R$ to be at most $r$. However, we keep $R>0$ for the sake of generality.}
    % Then we have that 
    % \begin{align}
    %     CC_\xi(R)&\leq \left(1 - \frac{x^{d+2} - x}{ dx - (d+1))}\right)\cdot R \frac{\partial(B_1)}{\sqrt{\det(\Lambda)}}\btheta^d_{R}  \nonumber\\&+ R\cdot P_d(\btheta_R).
    % \end{align}
  Then,
    \begin{align}
        CC_\X\leq \left(1 - \frac{x^{d+2} - x}{ dx - (d+1))}\right) \cdot 4\delta \cdot  \btheta_r^d + r \cdot P_d(\btheta_r),
    \end{align}
    where \kiril{$x:=?$ Let's also use a different notation for $x$, e.g., $\xi$}
\end{thm}
\begin{proof}
  We improve the naive bound in Equation~\eqref{eq:cc_naive} by partitioning the $r$-ball into annuli. Let us start with a simple example. Fix $0<r_1<
  r$, and define $\btheta_{r'} := \frac{r'}{\beta}f_\Lambda$, and observe that 
\begin{align}
  CC_\X&\leq  r\cdot
\left|\X\cap (\B_{r}\setminus \B_{r_1})\right| + r_1\cdot
\left|\X\cap \B_{r_1}\right|\nonumber \\ & = r\left(|\X\cap \B_{r}|-|\X \cap \B_{r_1}|\right) + r_1 \left|\X\cap \B_{r_1}\right| \nonumber\\
& = r|\X\cap \B_{r}|+ (r_1-r) |\X\cap \B_{r_1}| \nonumber \\  
  & = r\frac{\partial(B_1)}{\sqrt{\det(\Lambda)}}\btheta^d_{r} +r P_d(\btheta_{r}) + (r_1-r) \frac{\partial(B_1)}{\sqrt{\det(\Lambda)}}\btheta^d_{r_1}\nonumber\\& + (r_1-r) P_d(\btheta_{r_1}) \nonumber
\\
& = \frac{\partial(B_1)}{\sqrt{\det(\Lambda)}}\theta^d\left(r^{d+1}+{r_1}^{d+1}-r{r_1}^{d}\right)\nonumber\\&+ r P_d(\btheta_{r}) + (r_1-r) P_d(\btheta_{r_1})\nonumber \\ & = \frac{\partial(B_1)}{\sqrt{\det(\Lambda)}}\theta^d\left(r^{d+1}+{r_1}^{d+1}-r{r_1}^{d}\right)+ r P_d(\btheta_{r}), \label{eq:CC1}
\end{align}
where the sample complexity bound in Equation~\eqref{eq:sample_complexity} is used. For simplicity, we upper-bound throughout the error term with $r P_d(\btheta_{r})$.
Next, we optimize the value $r_1$ to minimize the expression in Equation~\eqref{eq:CC1}.

Consider the function $f(r_1)=r^{d+1}-r r^d_1 + r^{d+1}_1$. We look for the minimum of $f(r_1)$ by requiring that
\begin{align*}
            f'(r_1)=-r dr_1^{d-1}+(d+1)r_1^d=0,
\end{align*}
which yields the value $r^*_1:=\frac{d}{d+1}r$. This value is  a minimum since
\begin{align*}
 f^{(2)}(r_1)|_{r_1^*}=&\left(-r(d-1)r_1^{d-2}+d(d+1)r_1^{d-1}\right)|_{r_1^*}\\
        =&r^{d-1}\left(\frac{d^d}{(d+1)^{d-2}}-\frac{d^{d-2}(d-1)}{(d+1)^{d-2}}\right)\\
        =&r^{d-1}d^{d-2}\frac{d^2-d+1}{(d+1)^{d-2}},
    \end{align*}
    and we know that $d^2-d+1>0$ for all $d\geq 2$.%, then $r_1=\frac{d}{d+1}r$ indeed minimizes $f(r_1)$.
    
  
  %   We will use the above expression to upper-bound the number of points in the annulus $\{r_{i+1}\leq \|x\| \leq r_i\}$: %which we would then multiply by $r_i$ to obtain an upper-bound of the distances of points within it. In particular,
% %we can then say that the number of samples we have is approximately \itai{what is the right "approx" here?} the difference of the aforementioned expressions. Recalling that we need to work with $r_i'=\frac{f_\Lambda}{\beta}r_i$ due to rescaling, we get
%     \begin{align*}
%       \left|\X\cap (\B_{r_i}\setminus \B_{r_{i+1}})\right| &=O\left(\frac{1}{d}\left(\frac{2\pi e}{d}\right)^{\frac{d}{2}}(\btheta^d_{r_i}-\btheta^d_{r_{i+1}}) + \btheta^{d-2}_{r_i} - \btheta^{d-2}_{r_{i+1}}\right)\\ &=O\left(\left(\frac{f_\Lambda}{\beta}\right)^{d-2}\left(\underbrace{\frac{1}{d}\left(\frac{2\pi e}{d}\right)^{\frac{d}{2}}\left(\frac{f_\Lambda}{\beta}\right)^2}_{=:\gamma}\left(r_{i}^d-r_{i+1}^d\right)+\left(r_{i}^{d-2}-r_{i+1}^{d-2}\right)\right)\right).      
%     \end{align*}
%     For each such annulus, the maximal radius is $r_i$, and so the sum of distances at the annulus is at most 
% \begin{align} r_i\cdot
% \left|\X\cap (\B_{r_i}\setminus \B_{r_{i+1}})\right|=O\left(\left(\frac{f_\Lambda}{\beta}\right)^{d-2}\left(\gamma\left(r_i^{d+1}-r_ir_{i+1}^d\right)+\left(r_i^{d-1}-r_ir_{i+1}^{d-2}\right)\right)\right).
% \end{align}
% Consequently, we can use the above bound to compute. 
% \begin{align*}
%   CC_\X(r)&\leq \sum_{i=0}^{n-1} r_i\cdot
% \left|\X\cap (\B_{r_i}\setminus \B_{r_{i+1}})\right| + r_n\cdot
% \left|\X\cap \B_{r_n}\right|. %\\ &=
% %\sum_{i=0}^nO\left(\left(\frac{f_\Lambda}{\beta}\right)^{d-2}\left(\gamma\left(r_i^{d+1}-r_ir_{i+1}^d\right)+\left(r_i^{d-1}-r_ir_{i+1}^{d-2}\right)\right)\right) + O\left(\left(\frac{f_\Lambda}{\beta}\right)^{d-2}\left(\gamma r_i^{d+1}+r_i^{d-1}\right)\right)
% \end{align*}

% Next, we derive a heuristic for specifying the radii $r_i$ to minimize the expression $CC_\X(r)$. For that purpose, we will start with the simple case where $n=1$. Observe that
% \begin{align*}
%   CC_\X(r)&\leq  r_1\cdot
% \left|\X\cap (\B_{r}\setminus \B_{r_{1}})\right| + r_1\cdot
% \left|\X\cap \B_{r_1}\right| \\
%   & =O\left(\left(\frac{f_\Lambda}{\beta}\right)^{d-2}\left(\gamma\left(r^{d+1}-rr_{1}^d+r_1^{d+1}\right)+\left(r^{d-1}-rr_{1}^{d-2}+r_1^{d-1}\right)\right)\right).
% \end{align*}

Now, we apply the above line of reasoning in a recursive manner by considering a sequence of $k+1\geq 2$ radii ${0<r_k<\ldots<r_0=r}$ where $r_i:=\td^i r$, where $\td:=\frac{d}{d+1}$. This leads to the bound
\begin{align}
\label{eq:cc_eval}
CC_\X(r)&\leq \sum_{i=0}^{k-1}r_i |\X\cap (\B_{r_i}\setminus \B_{r_{i+1}})| + r_k|\X\cap \B_{r_k}|\nonumber\\
  &= \sum_{i=0}^{k-1}r_i\left(|\X\cap \B_{r_i}|- |\X\cap \B_{r_{i+1}}|\right)+ r_k|\X\cap \B_{r_k}| \nonumber\\
  &= r_0|\X\cap \B_{r_0}| + \sum_{i=1}^{k}(r_i - r_{i-1})|\X\cap \B_{r_i}| \nonumber\\
  & =r_0\left(\frac{\partial(B_1)}{\sqrt{d}}\btheta^d_{r_0} +\P_d(\btheta^{d-2}_{r_0})\right) \nonumber\\&+ \sum_{i=1}^{k}(r_i - r_{i-1}) \left(\frac{\partial(B_1)}{\sqrt{d}}\btheta^d_{r_i} +\P_d(\btheta^{d-2}_{r_i})\right) \nonumber\\
  &= \frac{\partial(B_1)}{\sqrt{d}} \left(\underbrace{r_0 \btheta^d_{r_0} + \sum_{i=1}^k(r_i-r_{i-1}) \btheta^d_{r_i}}_{:=\gamma(d)}\right) \nonumber\\&+ \P_d\left(\underbrace{r_0\btheta^{d-2}_{r_0} + \sum_{i=1}^{k}(r_i - r_{i-1}) \btheta^{d-2}_{r_i}}_{:=\gamma(d-2)}\right).
\end{align}

Next, we develop the expression $\gamma(N)$ above for some general $N\in\mathbb{N}$ by substituting $r_i=\td^i r$ and $\btheta_{r_i}= r_i\btheta_{r}/r$: 
\begin{align}
  \gamma(N) &=r \btheta^N_{r} + \sum_{i=1}^k(r_i-r_{i-1}) r_i^d\frac{\btheta^N_{r}}{r^d} \nonumber\\
  & = r \btheta^N_{r} + \sum_{i=1}^kr\td^{i-1}(\td-1) \td^{di} r^d\frac{\btheta^N_{r}}{r^d} \nonumber\\ 
  &=  r \btheta^N_{r} + \sum_{i=1}^kr (\td-1) \td^{Ni+ i -1} \btheta^N_{r} \nonumber\\ 
  &=   r \btheta^d_{r} \left(1 + \sum_{i=1}^k (\td-1) \td^{Ni+ i -1} \right)\nonumber\\
  &= r \btheta^N_{r} \left(1 + \frac{\td-1}{\td}\sum_{i=1}^k \td^{(N+1)i} \right)\nonumber\\
  &= r \btheta^N_{r} \left(1 + \frac{\td-1}{\td}\frac{\left(\td^{N+1}\right)^{k+1} - \td^{N+1}}{\td^{N+1} - 1} \right)\nonumber\\
  &= r \btheta^N_{r} \left(1 + \td^N(\td-1)\frac{\left(\td^{N+1}\right)^k - 1}{\td^{N+1} - 1} \right).\nonumber\\
  % & = r \btheta^d_{r} + \sum_{i=1}^kr\td^{i-1}(\td-1) \td^{di} r^d\frac{\btheta^d_{r}}{r^d} \\ &  =  r \btheta^d_{r} + \sum_{i=1}^kr (\td-1) \td^{di+ i -1} \btheta^d_{r} \\ & =   r \btheta^d_{r} \left(1 + \sum_{i=1}^k (\td-1) \td^{di+ i -1} \right)\\
\end{align}

Taking $k=d$ results in $r_k=(\frac{d}{d+1})^dr\approx\frac{1}{e}r$ . To use the sample set analysis, we need a large enough $r$ value, so assuming the original $r$ is large enough, we can deduce safely that $\frac{r}{e}$ is also large enough. Notice also that $\td - 1 = \frac{-1}{d+1}$, so returning to our expression, we get
\begin{align*}
      &= r \btheta^N_{r} \left(1 - \frac{\td^N\left(\td^{d(N+1)} - 1\right)}{(d+1)(\td^{N+1} - 1)}\right).
      % &= r \btheta^d_{r} \left(1 - \frac{x\left(x^{d+1} - 1\right)}{(d+1)(\td x - 1)}\right)\nonumber\\
      % &= r \btheta^d_{r} \left(1 - \frac{x^{d+2} - x}{ dx - (d+1))}\right).
\end{align*}
Notice that $\td < 1$. Therefore, $\td^{d(N+1)}-1 < 0$ and $\td^{N+1} - 1 < 0$, so our expression in the parenthesis is less than 1---suggesting an improvement on the trivial bound with $\gamma(N)$.
Let $x:=\td^d$, we get:
\begin{align*}
    \gamma(d)&=r \btheta^d_{r} \left(1 - \frac{\td^d\left(\td^{d(d+1)} - 1\right)}{(d+1)(\td^{d+1} - 1)}\right)\\
    &= r \btheta^d_{r} \left(1 - \frac{x\left(x^{d+1} - 1\right)}{(d+1)(\td x - 1)}\right)\nonumber\\
    &= r \btheta^d_{r} \left(1 - \frac{x^{d+2} - x}{ dx - (d+1))}\right),\\
    \gamma(d-2)&=r \btheta^{d-2}_{r} \left(1 - \frac{\td^d\left(\td^{d(d-1)} - 1\right)}{(d+1)(\td^{d-1} - 1)}\right)\\
    &= r \btheta^{d-2}_{r} \left(1 - \frac{x\left(x^{d-1} - 1\right)}{(d+1)(\frac{x}{\td} - 1)}\right)\nonumber\\
    &= r \btheta^{d-2}_{r} \left(1 - \frac{x^d - x}{ \frac{(d+1)^2}{d}x - (d+1))}\right)\nonumber\\
    &= r \btheta^{d-2}_{r} \left(1 - \frac{d(x^d - x)}{ (d+1)^2x - d(d+1))}\right) \nonumber\\
    &= r \btheta^{d-2}_{r} \left(1 - \frac{d}{d+1}\frac{x^d - x}{ (d+1)x - d}\right).
\end{align*}
Finally, we return to our original upper bound in~\ref{eq:cc_eval}, getting
\begin{align*}
    CC_\X(r)&\leq \left(1 - \frac{x^{d+2} - x}{ dx - (d+1))}\right)\cdot r \frac{\partial(B_1)}{\sqrt{\det(\Lambda)}}\btheta^d_{r}  \\&+ \P_d\left(\left(1 - \frac{d(x^d - x)}{ (d+1)^2x - d(d+1))}\right)\cdot r \btheta^{d-2}_{r} \right)
\end{align*}
with $x:=\td^d, \td:=\frac{d}{d+1}$.

% The general expression we get is
%     \begin{align*}
%         r_i^{D+1} - r_ir_{i+1}^D=&
%         \left(\left(\frac{D}{D+1}\right)^ir\right)^{D+1} - \left(\left(\frac{D}{D+1}\right)^ir\right)\left(\left(\frac{D}{D+1}\right)^{i+1}r\right)^D\\
%         =& r^{D+1}\left[\left(\left(\frac{D}{D+1}\right)^i\right)^{D+1} - \frac{D+1}{D}\left(\left(\frac{D}{D+1}\right)^{i+1}\right)^{D+1}\right]\\
%         =& r^{D+1}\left[\left(\left(\frac{D}{D+1}\right)^i\right)^{D+1} -\frac{D+1}{D}\left(\left(\frac{D}{D+1}\right)^i\right)^{D+1}\left(\frac{D}{D+1}\right)^{D+1}\right]\\
%         =& r^{D+1}\left(\left(\frac{D}{D+1}\right)^i\right)^{D+1}\left(1-\left(\frac{D}{D+1}\right)^D\right)
%     \end{align*}
%     After simplifying this, recall that the approximation for the number of samples in a ball is true for radius values that are big enough. Therefor, we need to start from $i=k$ big enough such that $\left(\frac{D}{D+1}\right)^ir$ is still a big enough radius. Dotice that for $i=D$ we get $\left(\frac{D}{D+1}\right)^D\geq\frac{1}{e}$, so we can safely use $i=D,r_D\approx0.36r$ up until even $i=2D,r_{2D}\approx0.13r$. We now sum over all valid annulus, getting
%     \begin{align*}
%         &\sum_{i=0}^{i=k}r^{D+1}\left(\left(\frac{D}{D+1}\right)^i\right)^{D+1}\left(1-\left(\frac{D}{D+1}\right)^D\right)\\
%         =&r^{D+1}\left(1-\left(\frac{D}{D+1}\right)^D\right)\sum_{i=0}^{i=k}\left(\left(\frac{D}{D+1}\right)^{D+1}\right)^i\\
%         =& r^{D+1}\left(1-\left(\frac{D}{D+1}\right)^D\right)\frac{\left(\frac{D}{D+1}\right)^{(k+1)(D+1)} - 1}{\left(\frac{D}{D+1}\right)^{D+1} - 1}\\
%         =& r^{D+1}\frac{1-\left(\frac{D}{D+1}\right)^D}{1-\left(\frac{D}{D+1}\right)^{D+1}}\left(1-\left(\frac{D}{D+1}\right)^{(k+1)(D+1)}\right),
%     \end{align*}
%     We now add the innermost $r_k$-ball, in addition to the annulii, getting
%     \[
%         r^{D+1}\frac{1-\left(\frac{D}{D+1}\right)^D}{1-\left(\frac{D}{D+1}\right)^{D+1}}\left(1-\left(\frac{D}{D+1}\right)^{(k+1)(D+1)}\right)+\left(\frac{D}{D+1}\right)^{k(D+1)}r^{D+1}:=r^{D+1}a_{D,k},
%     \]
    % with letting $a_{D,k}$ be the entire expression without the $r^{D+1}$ part. Let us use this on our original expression
    % \begin{align*}
    %     I(r)=&\frac{1}{d}\left(\frac{2\pi e}{d}\right)^{\frac{d}{2}}\left(\frac{f_\Lambda}{\beta}\right)^{d+1}r^{d+1}a_{D,k} + \left(\frac{f_\Lambda}{\beta}\right)^{d-1}r^{d-1}a_{D-2,k}
    % \end{align*}
\end{proof}

\begin{figure}[thb]
\centering  
\includegraphics[width=0.9\columnwidth]{Images/annuli_bound.png}
\caption{Theoretical sample limit improvement factor using the annuli method. \kiril{Change orientation of improvement factor to vertical.}}
\label{fig:annuli_bound}
\end{figure}

We can see in~\Cref{fig:annuli_bound} the improvement term of the main term as a function of the dimension: notice that the improvement rate diminishes as $d$ gets larger.%Comparatively, the trivial bound would've given us:
%\[
%    CC_\X(r)\leq r \frac{\partial(B_1)}{\sqrt{d}}\btheta^d_{r} + \Theta\left(r \btheta^{d-2}_{r} \right)
%\]
% \begin{figure*}[!h]
%   \centering
%   \subfloat["H" map]{
%     \includegraphics[width=0.3\textwidth]{Images/Hmap_basic.png}
%     \label{fig:exp_3body:hmap}}
%   \hfil
%   \subfloat["Random polygons" map]{
%     \includegraphics[width=0.3\textwidth]{Images/rndpoly_basic.png}
%     \label{fig:exp_3body:rndpoly}}
%   \caption{The scenarios we used to test our sample set, in each map we wanted each disk-robot to switch places with the next neighbor. \kiril{Add more dimensions to the left and right plots.}}
%   \label{fig:exp_3body}
% \end{figure*}

\kiril{Note to self: revise this paragraph.} To compare these values with a theoretical "better" one, a simulation was run with the following algorithm: 
\begin{enumerate}
    \item Assume $d=6,r_0=1, r_D=\left(\frac{D}{D+1}\right)^{k}$.
    \item In addition to these two radii, add $D-2$ more concentric circles of random radius values between the values $r_0, r_D$.
    \item For this random division, calculate the fitting $r^{d+1},r^{d-1}$ improvement parameters (we get them due to setting $r=1$).
\end{enumerate}
After running this process for 1000 iterations, the best parameters we got were $0.881, 0.821$, for $r^{d+1},r^{d-1}$ (respectively). This suggests that while there is room for improvement in this method, it is close enough to the best improvement we can get in the method of "layered approximation."
% \subsection*{A bit of intuition on the achieved upper bound}
% Notice that asymptotically, as $d$ gets very large, the term $\left(1+\frac{1-e^{-d}}{d}\right)$ goes very quickly to $1$. So at higher $d$ values, we are effectively left with the original sample sizes, only now times the rescaled radius again, getting $O(radius\cdot \#samples)$.
% % \[
% %     I\left(r\right)\approx O\left(\left(\sum_i\|e_i\|^2\right)\btheta^{d-2}\left(\frac{\btheta}{r \left(d-1\right)}+1\right)\right).
% % \]
% % Seeing as $\btheta>1$ and $d$ is high, we can ignore the $+1$ term, and get
% % \[
% %     I\left(r\right)\approx O\left(\frac{\sum_i\|e_i\|^2}{r\left(d-1\right)}\btheta^{d-1}\right),
% % \]
% % and because, as we will see below, we deal with lattices such that ${\sum_i\|e_i\|^2=O\left(d\right)}$, we end up with
% % \[
% %     I\left(r\right)\approx O\left(\frac{d}{r\left(d-1\right)}\btheta^{d-1}\right)= O\left(\frac{1}{r}\btheta^{d-1}\right).
% % \]
% % Recall that in theorem~\ref{general_sample_complexity} our dominant term for evaluating the number of samples is $\left(\btheta\right)^{d-2}$. Expecting an average distance of $c\btheta$ for points in the sphere (
% Looking at random points, we have an expected distance from the center of $\frac{n}{n+1}r$, so also with random points we "expect" to get more or less $O(\frac{n}{n+1}\cdot radius\cdot \#samples)=O(radius\cdot \#samples)$, which is similar to our term, suggesting that our upper bound is at least of the optimal order.
% \itai{Next part is irrelevant with this new computation. with this, it just becomes a direct extension of the sample-complexity section calculations.}
% % our total distance for a group of points is 
% % \[
% %     I\left(r\right)\approx c\btheta \cdot \left(\btheta\right)^{d-2}=O\left(\btheta\right)^{r-1},
% % \]
% % which is very similar to the type of term we managed to get. The specific complexity values for the lattices are not significantly different from this intuition, but it is important to show it rigorously.

%Next, we perform experiments to check the effectiveness of our lattices, compared to each other and to other sample sets.

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:

